Induced Cycles and Paths Are Harder Than You Think

The goal of the paper is to give fine-grained hardness results for the Subgraph Isomorphism (SI) problem for fixed size induced patterns $H$, based on the $k$-Clique hypothesis that the current best algorithms for Clique are optimal. Our first main result is that for any pattern graph $H$ that is a {\em core}, the SI problem for $H$ is at least as hard as $t$-Clique, where $t$ is the size of the largest clique minor of $H$. This improves (for cores) the previous known results [Dalirrooyfard-Vassilevska W. STOC'20] that the SI for $H$ is at least as hard as $k$-clique where $k$ is the size of the largest clique {\em subgraph} in $H$, or the chromatic number of $H$ (under the Hadwiger conjecture). For detecting \emph{any} graph pattern $H$, we further remove the dependency of the result of [Dalirrooyfard-Vassilevska W. STOC'20] on the Hadwiger conjecture at the cost of a sub-polynomial decrease in the lower bound. The result for cores allows us to prove that the SI problem for induced $k$-Path and $k$-Cycle is harder than previously known. Previously [Floderus et al. Theor. CS 2015] had shown that $k$-Path and $k$-Cycle are at least as hard to detect as a $\lfloor k/2\rfloor$-Clique. We show that they are in fact at least as hard as $3k/4-O(1)$-Clique, improving the conditional lower bound exponent by a factor of $3/2$. Finally, we provide a new conditional lower bound for detecting induced $4$-cycles: $n^{2-o(1)}$ time is necessary even in graphs with $n$ nodes and $O(n^{1.5})$ edges.

==> intro.tex <==



A fundamental problem in graph algorithms, Subgraph Isomorphism (SI) asks, given two graphs $G$ and $H$, does $G$ contain a subgraph isomorphic to $H$? 
While the problem is easily NP-complete, many applications only need to solve the poly-time solvable version in which the pattern $H$ has constant size; this version of SI is often called Graph Pattern Detection and is the topic of this paper. 
%Then if $G$ has $n$ vertices and $H$ has $k=O(1)$ vertices, even the brute-force algorithm runs in polynomial time $O(n^k)$.

The main motivation for this paper is the following intriguing question:
\begin{center}{\em What makes some patterns easier to detect than others}?\end{center}

There are two versions of SI: {\em induced} and not necessarily induced, {\em non-induced} for short. In the induced version, the copy of $H$ in $G$ must have both edges and non-edges preserved, whereas in the non-induced version only edges need to carry over, and the copy of $H$ in $G$ can be an arbitrary supergraph of $H$.
It is well known that the induced version of $H$-pattern detection for any $H$ of constant size is at least as hard as the non-induced version (see e.g. \cite{stoc-paper}), and that often the non-induced version of SI has faster algorithms (e.g. the non-induced $k$-independent set problem is solvable in constant time). Thus, when addressing SI, we need to be specific about the version we consider.


It is well-known that the SI problem (induced and non-induced) for any $k$-node pattern $H$ in $n$-node graphs for constant $k$, can be reduced to detecting a $k$-clique in an $O(n)$ node graph (see \cite{nevsetvril1985complexity}). Thus the hardest pattern to detect is $k$-clique.

When $k$ is divisible by $3$, the fastest known algorithm \cite{nevsetvril1985complexity} for $k$-clique runs in $O(n^{\omega k/3})$ time, where $\omega<2.37286$ \cite{almanv21} is the matrix multiplication exponent. For $k$ not divisible by $3$, the best running time is achieved via rectangular matrix multiplication, and is 
 $C(n,k):=O(n^{\omega(\lfloor k/3\rfloor,\lceil k/3\rceil,\lceil (k-1)/3\rceil)})$ time, where $\omega(a,b,c)$ is the exponent of multiplying an $n^a\times n^b$ by an $n^b\times n^c$ matrix.


The $k$-clique running time $C(n,k)$ is the fastest known running time for many other $k$-node patterns.
Nevertheless, some patterns are easier to detect than $k$-clique. This is especially true in the non-induced case (e.g. \cite{alon1995color,KowalukLL13}). For instance, $k$-paths, $k$-cycles, and more generally patterns of bounded treewidth can be found in $2^{O(k)}\textrm{poly}(n)$ time via the color-coding method~\cite{alon1995color}, where the exponent of the polynomial in $n$ depends on the treewidth of $H$ but not on $k$. 

In the induced case, many patterns are also easier than $k$-clique, e.g. for $k=3,4,5,6$, any $H$ that is not the $k$-independent set or the $k$-clique can be found in the current best running time $C(n,k-1)$ for $(k-1)$-clique \cite{williams2014finding,stoc-paper}.
For $k\geq 7$, Bl\"{a}ser et al.~\cite{BlaserKS18} showed the weaker result that all $k$-node $H$ that are not the clique or independent set can be detected in $O(n^{k-1})$ time ``combinatorially'', whereas the best known ``combinatorial''\footnote{``Combinatorial" is not well-defined, but it is a commonly used term to denote potentially practical algorithms that avoid the generally impractical Strassen-like methods for matrix multiplication.} algorithms for $k$-clique run in $n^{k-o(1)}$ time.



This $k$-clique running time has remained unchallenged since the 1980s, and a natural hardness hypothesis has emerged (see e.g. \cite{vsurvey}):

\begin{hypothesis}[$k$-clique Hypothesis]
On a word-RAM with $O(\log n)$ bit words,
for every constant $k\geq 3$, $k$-clique  requires $n^{\omega(\lfloor k/3\rfloor,\lceil k/3\rceil,\lceil (k-1)/3\rceil)-o(1)}$ time.
\end{hypothesis}

A ``combinatorial'' version of the hypothesis states that the best combinatorial algorithm for $k$-clique runs in $n^{k-o(1)}$ time. For induced pattern detection for patterns of size $k\ge 8$, the best algorithm for almost all of the patterns has the same running time as $k$-clique detection\footnote{There are faster algorithms for $k\le 6$, and for each larger $k$ ?? have identified a few patterns that can be detected faster than $k$-clique detection running time}. If we only resort to combinatorial algorithms there is a slight improvement: any pattern that is not a clique or independent set can be detected in $O(n^{k-1})$ time \mina{cite}. The best algorithm for the non-induced pattern detection is the color-coding algorithm of Alon, Yuster and Zwick \mina{cite} from almost 30 years ago that gives a running time of $O(n^{t+1})$ if $t$ is the treewidth of the pattern.  The lack of any significant progress in algorithmic results suggest that we must look for strong lower bounds for the pattern detection problem.  

As $k$-clique is the hardest $k$-node pattern, it is natural to compare the SI problem for other patterns to the SI problem for $k$-clique (see e.g. \cite{stoc-paper,FloderusKLL15}). If $k$-clique detection in $n$-node graphs can be efficiently reduced to the the SI problem for a pattern $H$ in $O(n)$-node graphs, then under the above hypothesis, $H$-pattern detection requires $C(n,k)^{1-o(1)}$ time. Thus we get a {\em fine-grained} lower bound on the running time.

A fine-grained reduction from $k$-clique to $H$-detection has other consequences\footnote{Note that here $H$ is not necessarily of size $k$.}. For instance, since under the Exponential Time Hypothesis (ETH), $k$-clique requires $n^{\Omega(k)}$ time, the same lower bound would apply to $H$-detection. However, such a lower bound is not fine-grained, and only makes sense for families of patterns on $k$ vertices (where $k$ can grow; it wouldn't make sense for fixed patterns $H$).

In this paper we present several fine-grained lower bounds under the $k$-clique Hypothesis, and other well-established hypotheses such as ETH. \mina{add something like: our results are not tight yet, but since it is even unclear what dictates the exact complexity of patterns, any imporovement on lower bounds for any class of graphs is important. }

% (*** maybe put this later ***)
% We note that some seemingly stronger conditional lower bounds (e.g. \cite{ManurangsiRS21}) have been published for some of our results. However, these results are under a much less established hypothesis.


\section{Our results}

%\mina{the story starts here.}
%Our techniques imply improved hardness for arbitrary $k$-node subgraphs as well.
Dalirrooyfard, Vuong and Vassilevska W. \cite{stoc-paper} related the hardness of subgraph pattern detection to the size of the maximum clique or the chromatic number of the pattern.
In particular, they showed that if $H$ has chromatic number $t$, then under the Hadwiger conjecture, $H$ is at least as hard to detect as a $t$-clique. 

The Hadwiger conjecture basically states that the chromatic number of a graph is always at most the largest size of a clique minor of the graph. As the result of \cite{stoc-paper} was already assuming the Hadwiger conjecture, one might wonder if it can be extended to show that every pattern $H$ is at least as hard to detect as an $\eta$-clique, where $\eta$ is the size of the largest {\em clique minor} of $H$.

We first note that such an extension is highly unlikely to work for non-induced patterns: the four cycle $C_4$ has a $K_3$ (triangle) minor, but a non-induced $C_4$ has an $O(n^2)$ time detection algorithm that does not use matrix multiplication, whereas any subcubic triangle detection algorithm must use (Boolean) matrix multiplication \cite{focsy}. Thus any extension of the result that shows clique minor sized clique hardness would either only work for certain types of non-induced graphs, or will need to only work in the induced case.

Here we are able to show that $H$-subgraph pattern detection, even in the non-induced case, is at least as hard as $\eta$-clique, where $\eta$ is the largest clique minor size of $H$, as long as $H$ is a special type of pattern called a {\em core}. Cores include many patterns of interest, including the complements of cycles of odd length.
 We also give several other hardness results, such as removing the dependence on the Hadwiger conjecture from some of the results of \cite{stoc-paper} with only a slight loss in the lower bound. 

We call a subgraph $C$ of a graph $H$ a {\em core} of $H$ if there is a homomorphism $H\rightarrow C$ but there is no homomorphism $H\rightarrow C'$ for any proper subgraph $C'$ of $C$. 
Hell and Ne{\v{s}}et{\v{r}}il~\cite{hell1992core} showed that every graph has a unique core (up to isomorphism), and the core of a graph is an {\em induced} subgraph. We denote the core of a graph $H$ by $core(H)$. A graph which is its own core is called simply a {\em core}.

We prove strong hardness results for pattern graphs that are cores, relating the hardness of detecting the pattern to the size of its maximum clique minor. We then relate the hardness of detecting arbitrary patterns to the hardness of detecting their cores.
%Our approach is similar to that of Dalirrooyfard, Duong Vuong and Vassilevska W.~\cite{stoc-paper} who related the hardness of pattern detection to the size of the maximum clique or the chromatic number of the pattern.

We begin with a theorem that shows hardness for detecting a ``partitioned'' copy of a pattern $H$. Here the vertex set of the host graph $G^*$ is partitioned into $k$ parts, and one is required to detect an induced copy of a $k$-node $H$ so that the image of the $i$th node of $H$ is in the $i$th part of the vertex set of $G^*$. This version of SI is often called Partitioned Subgraph Isomorphism (PSI).  Marx \cite{marx2007can} showed that under ETH, PSI for a pattern $H$ requires at least $n^{\Omega(tw(H)/\log{tw(H)})}$ time where $tw(H)$ is the treewidth of $H$. We give a more fine-grained lower bound for PSI. We provide a reduction from $\eta$-clique detection in an $n$ node graph to PSI for a graph $H$ in an $O(n)$ node host graph, for any $H$ with maximum clique minor of size  $\eta$.

\begin{restatable}{theorem}{psihardness}
\label{thm:psihardness} 
\textbf{(Hardness of PSI)} Let $H$ be a $k$-node pattern with maximum clique minor of size $\eta(H)$, and let $G$ be an $n$-node graph. Then one can construct a $k$-partite $O(n)$-node graph $G^*$ in $O(n^2)$ time such that $G^*$ has a colorful copy of $H$ if and only if $G$ has a clique of size $\eta(H)$.
\end{restatable}

Thus the hardness of Partitioned SI is related to the size of the largest clique minor.

To obtain a bound on the size of the maximum clique minor of any graph we use a result of Thomason \cite{thomason2001extremal} as follows: Let $c(t)$ be the minimum number such that every graph $H$ with $|E(H)|\ge c(t)|V(H)|$ has a $K_t$ minor. Then $c(t)=(\alpha+o(1))t\sqrt{\log{t}}$, where $\alpha\le 0.32$ is an explicit constant. Since for $t=\frac{|E(H)|/|V(H)|}{\sqrt{\log (|E(H)|/|V(H)|)}}$ the above inequality is true, we have the following corollary. 
\begin{corollary}
Let $H$ be a $k$-node $m$-edge pattern. Then the problem of finding a partitioned copy of $H$ in an $n$-node $k$-partite graph is at least as hard as finding a clique of size $\frac{m/k}{\sqrt{\log{m/k}}}$ in an $O(n)$-node graph.
\end{corollary}

Hence, for example if $m=ck^2$ for some constant $c$, then the PSI problem for $H$  cannot be solved in $n^{o\left({\frac{k}{\sqrt{\log{k}}}}\right)}$ time. Thus, for dense enough graphs, we 
improve the lower bound of $n^{\Omega(tw(H)/\log{tw(H)})}$ due to Marx \cite{marx2007can}, since $tw(H)\le k$.
% \mina{so we have $tw(H)=O(k)$ in this case: because $tw$ of any graph is at least the minimum degree of the graph, and so there is a subgraph $H'$ of $H$ having min degree $ck$, and since $tw(H)\ge tw(H')$, we have $tw(H)\ge ck$.}

% \mina{so for dense graphs, we improve the lower bound of Marx by $\sqrt{\log}$ in the exponent. Was he maybe asking if we can do that in his paper?}




%technique: The problem of having repeatedd vertices: color coding.
%\subsection{(Induced) subgraph isomorphism}
%Here we move to a generalization of the approach of \cite{stoc-paper} on giving lower bounds for SI. 
%The first hardness result on subgraph isomorphism with core patterns is by Marx \cite{marx2007can} where he showed that PSI and SI are equivalent on cores, and so using his PSI lower bound, by ETH detecting a core pattern $H$ in an $n$-node graph requires  $n^{\Omega{(tw(H)/\log{(tw(H)}))}}$ time where $tw(H)$ is the treewidth of $H$.  
%We give the first fine-grained hardness (correct term?) result on cores, using Theorem \ref{thm:psihardness}.
%From the equivalence of Subgraph Isomorphism and PSI on cores, we have the following hardness result on cores due to Theorem \ref{thm:psihardness}.


While Theorem~\ref{thm:psihardness} only applies to PSI, one can use it to obtain hardness for SI as well, as long as $H$ is a core. In particular, Marx~\cite{marx2007can} showed that PSI and SI are equivalent on cores. Thus we obtain:

\begin{restatable}{corollary}{corehardnessinsi}
\label{thm:core-hardness}
\textbf{(Hardness of cores in SI)} Let $G$ be an $n$-node $m$-edge graph and let $H$ be a $k$-node pattern with maximum clique minor of size $\eta(H)$. If $H$ is a core, then one can construct a graph $G^*$ with at most $O(n)$ vertices in $O(m+n)$ time such that $G^*$ has a subgraph isomorphic to $H$ if and only if $G$ has a $\eta(H)$-clique as a subgraph.
\end{restatable}

As the complements of odd cycles are cores with maximum clique minor of size $\floor{3k/4}$ \mina{check} for $C_k$ when $k$ is odd, we immediately obtain a lower bound of $C(n,\floor{3k/4})$ for $C_k$ detection. When $k$ is even, more work is needed.

% \mina{We use this result for getting better bounds for paths and cycles, where we modify this construction using new ideas, and those ideas might be useful for other pattern in future works. This is the main motivation for this theorem.}


% \mina{This result is similar to the simple case of theorem 2.1 in the stoc paper. That result says that if $H$ is $t$-chromatic, you can reduce $t$-clique detection to $H$-detection.

Corollary~\ref{thm:core-hardness} applies to the non-induced version of SI. We obtain a stronger result for the induced version in terms of the $k$ and the size of the largest clique subgraph.

\begin{restatable}{corollary}{corehardnessgeneral}
\label{cor:coreLB}
\textbf{(Hardness for induced-SI for cores)}
Let $H$ be a $k$-node pattern which is a core. Suppose that $w(H)$ is the size of the maximum clique in $H$. Then detecting $H$ in an $n$-node graph as an induced subgraph is at least as hard as detecting a clique of size $\max\{\ceil{\sqrt{(k+2w(H))/2}},\ceil{\sqrt{k/1.95}\}}$.
\end{restatable}


For comparison, the result of \cite{stoc-paper} shows that
 non-induced SI for any $k$-node $H$ is at least as hard as detecting a clique of size $\sqrt{k}$, but the result is conditioned on the Hadwiger conjecture. 
 Corollary \ref{cor:coreLB} is the strongest known clique-based lower bound result for $k$-node {\em core} $H$ that is not conditioned on the Hadwiger conjecture.

%Finally we improve this result for cycles of size $4t+1$ by a factor of $n^{0.5}$.

%Using the techniques in the proof of Theorem \ref{thm:core-hardness}, we conclude that induced-$C_k$ and induced-$P_k$ detection is at least as hard as $(\floor{\frac{3k}{4}}-2)$-clique detection, which improves the previous lower bound, saying that it is as hard as $k/2$-clique detection [stoc paper]. 

%To show hardness for general graphs, we define the notion of an "absolute core". $C$ is an absolute core of $H$ if there $C$ is a core graph and a subgraph of $H$ and if there is a homomorphism from $C$ to $C'$ which is a subgraph of $H$, then $C'$ and $C$ are isomorphic. 

Our next theorem relates the hardness of detecting a pattern to the hardness of detecting its core.

\begin{restatable}{theorem}{generalhardness}
\label{thm:general-hardness}
Let $G$ be an $n$-node $m$-edge graph and let $H$ be a $k$-node pattern. Let $C$ be the core of $H$. Then one can construct a graph $G^*$ with at most $O(n)$ vertices in $O(n^2)$ time such that $G^*$ has a subgraph isomorphic to $H$ if and only if $G$ has a subgraph isomorphic to $C$, with high probability\footnote{with probability $1/\poly{n}$}.
\end{restatable}

One consequence of Theorem~\ref{thm:general-hardness} and Corollary \ref{cor:coreLB} is that induced-SI for \emph{any} pattern $H$ of size $k$ is at least as hard as detecting a clique of size $\ceil{k^{1/4}/1.39}$. Note that this is the first lower bound for induced SI that is {\bf only} under the $k$-clique hypothesis.

\begin{restatable}{corollary}{inducedsihardnessone}\label{cor:inducedhardnessone}
\textbf{(Hardness of Induced-SI)}
For any $k$-node pattern $H$, detecting an induced copy of $H$ in an $n$-node graph is at least as hard as detecting a clique of size $\ceil{k^{1/4}/1.39}$ in an $O(n)$ graph.
\end{restatable}

We now consider some consequences under ETH.
Given Theorem~\ref{thm:general-hardness} and a result of  Marx\cite{marx2007can}, we are able to show that under ETH, there can be no $n^{o(\sqrt{k}/\log{k})}$ time algorithm for detecting any $k$-node $H$ as an induced subgraph of an $n$ node host graph. 

\begin{restatable}{corollary}{inducedsihardness} 
\label{cor:induced-si-hardness}
\textbf{(Hardness of Induced-SI)}
For any $k$-node pattern $H$, the problem of detecting an induced copy of $H$ in an $n$-node graph requires $n^{\Omega{(\sqrt{k}/\log{k})}}$ time under ETH. 
\end{restatable}

%\mina{add $n^{k^{1/4}}$ lower bound from cor 1.3 as a result without eth.}

Recall that
\cite{stoc-paper} shows that induced-SI for any $k$-node $H$ is at least as hard as $\sqrt k$-clique, and hence under ETH, needs $n^{\Omega\left(\sqrt k\right)}$ time.
However that result is
 \textbf{conditioned on the Hadwiger conjecture}.
 The above corollary gives a slightly weaker lower bound \textbf{independent} of the Hadwiger conjecture. 

\paragraph{Longer induced cycles and paths.}
We now focus on $k$-paths $P_k$ and $k$-cycles $C_k$ for larger $k$ and provide highly improved fine-grained lower bounds for their detection under the $K$-clique Hypothesis. The results can be viewed as relating how close induced paths and cycles are to cliques. Our techniques for proving our results can be of independent interest and can potentially be implemented to get stronger hardness results for other classes of graphs. 

\begin{table}[h]
\caption{Known upper and lower bounds for paths and cycles. The algorithms for $P_3$ and $C_3$ are folklore,  for $P_4$ from \cite{4path}, for $C_4$  from \cite{williams2014finding}, and for $C_k$ and $P_k$ for $k\geq 5$ from \cite{BlaserKS18}. The old lower bounds are all from \cite{FloderusKLL15}; our new lower bounds appear in Theorem~\ref{thm:hardnesscyclepath}.}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
Pattern & Runtime  & Lower Bound & Comb. Runtime & Comb. Lower Bound\\
\hline\hline
$P_3$, $P_4$ & $O(m+n)$   & & $O(m+n)$  & \\
\hline
$C_4$ & $\tilde{O}(n^\omega)$  &   & $O(n^3)$  & \\
\hline
$C_3$, $C_5,$ $P_5$ & $\tilde{O}(n^\omega)$   & $n^{\omega-o(1)}$  & $O(n^3)$  & $n^{3-o(1)}$ \\
\hline
$C_6,P_6$ & $C(n,4)$  & $n^{\omega-o(1)}$ & $O(n^4)$ & $n^{3-o(1)}$ \\
& $=O(n^{\omega(2,1,1)})$ &   &   & \\
\hline
$P_7$ & $C(n,6)$ & $n^{\omega-o(1)}$ & {\bf $O(n^{5})$} & $n^{3-o(1)}$ \\
  & $=O(n^{2\omega})$ &  &   &  \\
\hline
$C_7$ & $C(n,6)$ & \textcolor{red}{$C(n,5)$} {\bf [new]} & {\bf $O(n^{5})$} & \textcolor{red}{$n^{5-o(1)}$} {\bf [new]} \\
  & $=O(n^{2\omega})$ & $n^{\omega-o(1)}$  [old] &   & $n^{3-o(1)}$ [old] \\
\hline 
$C_k$, $P_k$, $k\geq 8$ & $C(n,k)$ & \textcolor{red}{$C(n,\lfloor 3k/4\rfloor-2)$} {\bf [new]} & $O(n^{k-2})$  & \textcolor{red}{$n^{\lfloor3k/4\rfloor-2-o(1)}$} {\bf [new]}\\
$C_k$, odd $k$ & $C(n,k)$ & \textcolor{red}{$C(n,\lfloor 3k/4\rfloor)$} {\bf [new]} & $O(n^{k-2})$  & \textcolor{red}{$n^{\lfloor3k/4\rfloor-o(1)}$} {\bf [new]}\\
 &   & $C(n,\lceil k/2 \rceil)$  [old] & & $n^{\lceil k/2 \rceil-o(1)}$ [old]\\
\hline
\end{tabular}
\label{tab:paths}
\end{table}

%$C(n,5)\leq n^{4.09}$, $C(n,6)\leq n^{4.75}$

The fastest known algorithms for finding induced cycles or paths on $k$ nodes can be found in Table \ref{tab:paths}. For larger $k$, the best known algorithms are either the $k$-clique running time $C(n,k)$, or an $O(n^{k-2})$ time combinatorial algorithm by \cite{BlaserKS18}. For $k\leq 7$, slightly faster algorithms are known.

The best known conditional lower bounds so far \cite{FloderusKLL15} under the $k$-clique hypothesis stem from the fact that the complement of $C_k$ contains a $\lfloor k/2 \rfloor$-clique, and the complement of $P_k$ contains a $\lceil k/2\rceil$-clique.
These lower bounds show that the best known running time of $O(n^\omega)$ for $C_5$ and $P_5$ are likely optimal. Unfortunately, for larger $k$, these lower bounds are far from the best known running times.

We obtain polynomially higher lower bounds, raising the lower bound exponent from roughly $k/2$ to roughly $3k/4$.

%$(\floor{\frac{3k}{4}}-2)$-clique detection.
\begin{restatable}{theorem}{hardnesscyclepath}
\label{thm:hardnesscyclepath}
\textbf{(Hardness of $P_k$ and $C_k$)}
Let $H$ be the complement of a $P_k$ or the complement of a $C_k$. Suppose that $t$ is the size of the maximum clique minor of $H$. Then the problem of detecting $H$ in an $O(n)$-node graph is at least as hard as finding a $(t-2)$-clique in an $n$-node graph. If $k$ is odd, then detecting an induced $C_k$ is at least as hard as finding a $t$-clique.
\end{restatable}

The largest \emph{clique minor}\footnote{A $t$-clique minor of a graph $H$ is a decomposition of $H$ into $t$ connected subgraphs such that there is at least one edge between any two subgraphs.} of the complement of $C_k$ has size $\lfloor 3k/4\rfloor$ and of
the complement of 
$P_k$ has size at least $\lfloor (3k+1)/4\rfloor$.

Table \ref{tab:paths} summarizes our new lower bounds. Aside from obtaining a much higher conditional lower bound, our result shows that the best known combinatorial algorithm for $C_7$ detection is tight, unless there is a faster combinatorial algorithm for $5$-clique detection.
For algorithms that may be non-combinatorial, our lower bound for $C_7$ is at least $\Omega(n^{4.08})$ assuming that the current bound for $5$-clique is optimal.



\paragraph{The curious case of Four-Cycle.} \mina{maybe shorten this section? It is 3 pages right now so might divert the attention from the main results} After presenting multiple hardness results, to better understand the source of hardness of patterns we focus on the smallest pattern that we don't know the exact complexity of. The complexity of SI for all patterns on at most $3$ nodes in $n$-node graphs is well-understood. In the non-induced case, all patterns except for the triangle have an $O(n^2)$ time algorithm, whereas the triangle can be solved in $O(n^\omega)$ time, and this is believed to be optimal due to the known relationship between triangle detection and Boolean matrix multiplication \cite{focsy}. For induced patterns the same is true, except that the independent set on $3$ nodes has the same complexity as triangle detection.

\begin{figure}[ht]\centering
\includegraphics[width=8cm]{smallgraphs4}
\caption{A list of all induced $4$-node patterns with their best known algorithms and conditional lower bounds. All runtime bounds are within polylogarithmic factors, and can be found in \cite{williams2014finding} and \cite{EG04}. All lower bounds except for the new one in red are under the $k$-clique hypothesis for $k=3$ or $4$, and every lower bound $l$ as a function of $m$ or $n$ should be interpreted as $l^{1-o(1)}$. The new lower bound is under the $3$-uniform $4$-hyperclique hypothesis, only holds for $C_4$ and is in Theorem~\ref{thm:c4hard}. All upper and lower bounds are tight except that for $C_4$ and its complement.}
\label{fig:smallgraphs}
\end{figure}

We thus begin with the SI problem for $4$-node patterns. Table \ref{fig:smallgraphs} gives the best known algorithms and conditional lower bounds for induced SI for all $4$-node patterns. In the non-induced case, the change is that, except for the $4$-clique $K_4$, the diamond, co-claw and the paw whose runtimes and conditional lower bounds stay the same, all other patterns can be solved in $O(n^2)$ time.

All conditional lower bounds in Table \ref{fig:smallgraphs} are tight, except for the curious case of the induced $4$-Cycle $C_4$. Non-induced $C_4$ can famously be detected in $O(n^2)$ time (see e.g. \cite{non-induced-4cycle}). Meanwhile, the fastest algorithm for induced $C_4$ runs in $O(n^\omega)$ time (see e.g. \cite{williams2014finding}). It is completely unclear why matrix multiplication should be necessary for such a simple looking problem .


There is no non-trivial lower bound known for $C_4$ detection (except that one needs to read the graph), and obtaining a higher lower bound or a faster algorithm for $C_4$ has been stated as an open problem several times (see e.g. \cite{EschenHSS11}).

The induced $4$-cycle is the smallest pattern $H$ whose complexity is not tightly known, under any plausible hardness hypothesis.%\footnote{While the non-induced $4$-cycle doesn't have a tight lower bound either, since induced $C_4$-detection is at least as hard as non-induced $C_4$-detection, we focus on the induced version for obtaining a lower bound.}.

We make partial progress under the popular $3$-Uniform $4$-Hyperclique Hypothesis (see e.g. \cite{LincolnWW18,AbboudBDN18}) that postulates that hyperclique on $4$ nodes in an $n$ vertex $3$-uniform hypergraph cannot be detected in $O(n^{4-\eps})$ time for any $\eps>0$, in the word-RAM model of computation with $O(\log n)$ bit words. The believability of this hyperclique hypothesis is discussed at length in \cite{LincolnWW18} (see also \cite{AbboudBDN18}); one reason to believe it is that refuting it would imply improved algorithms for many widely-studied problems such as Max-$3$-SAT \mina{add ryan's paper from 2005}.

\begin{theorem}
Under the $3$-Uniform $4$-Hyperclique Hypothesis, there is no $O(m^{4/3-\eps})$ time or $O(n^{2-\eps})$ time algorithm for $\eps>0$ that can detect an induced $4$-cycle in an $n$-node, $m$-edge undirected graph.\label{thm:c4hard}
\end{theorem}

While our result conditionally rules out, for instance, a linear time (in the number of edges) algorithm for induced $C_4$, it does not rule out an $O(n^2)$ time algorithm for induced $C_4$ in dense graphs since the number of edges in the reduction instance is $\Theta(n^{3/2})$ in terms of the number of nodes $n$.
Ideally, we would like to have a reduction from triangle detection to induced $C_4$-detection, showing that $n^{\omega-o(1)}$ time is needed. Our Theorem does show this if $\omega=2$, but we would like the reduction to hold for any value of $\omega$, and for it to be meaningful in dense graphs. Note that even if $\omega=2$, a reduction from triangle detection would be meaningful, as it would say that a practical, combinatorial algorithm would be extremely difficult to obtain (or may not even exist).

Dalirrooyfard, Vuong and Vassilevska W. \cite{stoc-paper} showed that any pattern that contains a $k$-clique as a subgraph, is as hard as $k$-clique to detect. This doesn't help us with $C_4$, however, as the largest $k$-clique that it or its complement contain is an edge.


%$C_4$ does contain a $3$-clique minor (just collapse any of its edges). So one would hope to be able to exploit this in a reduction.

All known reductions from $k$-clique to SI for other patterns $H$ (e.g. \cite{FloderusKLL15,stoc-paper,Lin15}) work equally well for non-induced SI. In particular, in the special case when $H$ is bipartite, such as when $H=C_4$, the host graph also ends up being bipartite (e.g. \cite{Lin15} for bicliques, and  \cite{FloderusKLL15,stoc-paper} more generally).


%create ``$H$-partite'' graphs. The reduction starts from $G=(V,E)$ in which one wants to find a $k$-clique, and one creates a graph $G'$ that has an independent set of $n=|V|$ vertices for each of the vertices of $H$, and then edges between pairs of partitions that depend on the edges of $G$ and the desired encoding of a $k$-clique within $H$.

Unfortunately such reductions are doomed to fail for $C_4$. 
In bipartite graphs and more generally in triangle-free graphs, any non-induced $C_4$ is an induced $C_4$. Of course, any hypothetical fine-grained reduction from triangle detection to non-induced $C_4$ detection in triangle-free graphs, combined with the known $O(n^2)$ time algorithm for non-induced $C_4$ would solve triangle detection too fast.


The difference between induced $C_4$ and non-induced $C_4$ is that the latter calls for detecting {\em one} of the three patterns: $C_4,$ diamond or $K_4$. Could we have a reduction from triangle detection to induced $C_4$-detection in a graph that is {\em not} triangle-free, but is maybe $K_4$-free?
In order for such a reduction to work, it must be that detecting one of $\{C_4,K_4\}$ is computationally hard. 


We show that such reductions are also doomed. We provide a fast combinatorial algorithm that detects one of $\{C_4,H\}$ for any $H$ that contains a triangle. The algorithm in fact runs faster than the current matrix multiplication time, which (under the $k$-clique Hypothesis) is required for detecting any $H$ containing a triangle. Thus, any tight reduction from triangle detection to induced $C_4$ must create instances that contain {\em every} induced $4$-node $H$ that has a triangle.

\begin{restatable}{theorem}{cfourgeneral}
\label{thm:c4-general}
For any $4$-node graph $H$ that contains a triangle, 
detecting one of $\{C_4,H\}$ as an induced subgraph of a given $n$-node host graph can be done in $O(n^{7/3})$ time.
If $H$ is not a diamond or $K_4$, then $H$ or $C_4$ can be detected 
 $O(n^2)$ time.
\end{restatable}

The only case of Theorem \ref{thm:c4-general} that was known is that for $\{C_4,$ diamond $\}$. Eschen et al. \cite{EschenHSS11} considered the recognition of $\{C_4,$ diamond $\}$-free graphs and gave a combinatorial $O(n^{7/3})$ time algorithm for the problem. We show a similar result for every $H$ that contains a triangle. %\mina{todo: check this algorithm, if different from us: remove the word similar?}


The $C_4$ OR $H$ problem solved by our theorem above is a special case of the subgraph isomorphism problem in which we are allowed to return one of a {\em set of possible patterns}.  This version of SI is a natural generalization of non-induced subgraph isomorphism in which the set of patterns are all supergraphs of a pattern. This generalized version of SI
has practical applications as well. Often computational problems needed to be solved in practice are not that well-defined, so that for instance
you might be looking for something like a matching or a clique, but maybe you are okay with extra edges or some edges missing.
In graph theory applications related to graph coloring, one is often concerned with $\{H,F\}$-free graphs for various patterns $H$ and $F$ (e.g. \cite{KarthickM18,DabrowskiP18,DabrowskiDP17}). Recognizing such graphs is thus of interest there as well. 
 We call the problem of detecting one of {\em two} given induced patterns, ``Paired Pattern Detection''. 

Intuitively, if a set of patterns all contain a $k$-clique, then returning at least one of them should be at least as hard as $k$-clique. While this is intuitively true, proving it is not obvious at all. In fact, until recently \cite{stoc-paper}, it wasn't even known that if a single pattern $H$ contains a $k$-clique, then detecting an induced $H$ is at least as hard as $k$-clique detection. We are able to reduce $k$-clique in a fine-grained way to ``Subset Pattern Detection" for any subset of patterns that all contain the $k$-clique as a subgraph\footnote{Our reduction works in the weaker non-induced version and so it works for the induced version as well.}.

\begin{restatable}{theorem}{setdetectioncore}
\label{thm:set-detection-cor}
Let $S$ be a set of patterns such that every $H\in S$ contains a $k$-clique. Then detecting whether a given graph contains some pattern in $S$ is at least as hard as $k$-clique detection.
\label{thm:cliqueset}
\end{restatable}

While having a clique in common makes a subset of patterns hard to detect, intuitively, if several patterns are very different from each other, then detecting one of them should be easier than detecting each individually. We make this formal for Paired Pattern Detection in $n$ node graphs for $k\leq 4$ as follows:


\begin{itemize}
\item Paired Pattern Detection is in $O(n^2)$ time for {\em every pair} of $3$ node patterns. Moreover, for all but two pairs of patterns, it is actually in linear time.
\item Paired Pattern Detection for any pair of $4$-node patterns is in $\tilde{O}(n^\omega)$ time, whereas the fastest known algorithm for $4$-clique runs in supercubic, $O(n^{\omega(1,2,1)})$ time where $\omega(1,2,1)\leq 3.252$ \cite{GallU18} is the exponent of multiplying an $n\times n^2$ by an $n^2\times n$ matrix.
\item There is an $O(n^2)$ time algorithm that solves Paired Pattern Detection for $\{H,\bar{H}\}$ for any $4$-node $H$, where $\bar{H}$ is the complement of $H$. 
\end{itemize}

 The last bullet is a generalization of an old Ramsey theoretic result of Erd\"{o}s and Szekeres~\cite{erdosramsey}
made algorithmic by Boppana and Halld{\'{o}}rsson~\cite{BoppanaH92}. The latter shows that in linear time for any $n$-node graph, one can find either a $\log(n)$ size independent set or a $\log(n)$ size clique.
 Thus, for every constant $k$ and large enough $n$, there is a linear time algorithm that either returns a $k$-clique or an $I_k$.
 
We note that our generalization for $\{H,\bar{H}\}$ cannot be true in general for $k\geq 5$: both $H$ and its complement \footnote{For $k=5$, consider $H$ to be a triangle and two independent nodes. Both $H$ and its complement contain a triangle.} can contain a clique of size $\lceil k/2\rceil\geq 3$, and thus by our Theorem~\ref{thm:cliqueset}, their Paired Pattern Detection is at least as hard as $\lceil k/2\rceil$-clique, and thus is highly unlikely to have an $O(n^2)$-time algorithm.





\subsection{Related work}
There is much related work on the complexity of graph pattern detection in terms of the {\em treewidth} of the pattern. Due to the Color-Coding method of Alon, Yuster and Zwick \cite{alon1995color}, it is known that if a pattern $H$ has treewidth $t$, then detecting $H$ as a non-induced pattern can be done in $O(n^{t+1})$ time. Marx \cite{marx2007can} showed that there is an infinite family of graphs of unbounded treewidth so that under ETH, SI on these graphs requires $n^{\Omega(t/\log t)}$ time where $t$ is the treewidth of the graph. Recently, Bringmann and Slusallek \cite{BringmannS21} showed that under the Strong ETH, for every $\eps>0$, there is a $t$ and a pattern $H$ of treewidth $t$ so that detecting $H$ cannot be done in $O(n^{t+1-\eps})$ time. That is, for some patterns, $n^{t+1}$ is essentially optimal.

Manurangsi, Rubinstein and Schramm~\cite{ManurangsiRS21} formulated a brand new hypothesis on the hardness of planted clique. This new hypothesis implies many results that are not known to hold under standard hypotheses such as ETH or Strong ETH, including that for every $k$-node $H$, its induced pattern detection  problem requires $n^{\Omega(k)}$ time. While identifying new plausible hypotheses is sometimes worthwhile, our work strives to get results under standard widely-believed hypotheses, and to uncover combinatorial relationships between $H$-pattern detection and clique-detection, as cliques are the hardest patterns to detect.

Note that the results of Marx~\cite{marx2007can} and Bringmann and Slusallek~\cite{bringmann2021current} show hardness for specific classes of patterns, whereas the the results of Dalirrooyfard et al.~\cite{stoc-paper}, Manurangsi et al.~\cite{ManurangsiRS21} and this paper aim to determine hardness for \emph{any} $k$-node pattern. Our paper primarily focuses on giving lower bounds for fixed patterns such as $C_4,C_7$ etc., whereas the focus of \cite{ManurangsiRS21} is more asymptotic.


 

\subsection{Organization of the paper} In Section \ref{sec:technical-overview} we give a high level overview of our techniques, and a comparison to the past techniques. 
In Section \ref{sec:prelim} we give the necessary definitions. In Section \ref{sec:lower-bounds} we first state our hardness result for PSI (Theorem \ref{thm:psihardness}) in subsection \ref{sec:hardnessofpsi}, and then in subsection \ref{sec:corehardness} we state our hardness result for SI (Theorem \ref{thm:general-hardness}). Finally, in subsection \ref{sec:paths-and-cycles} we show hardness for paths and cycles (Theorem \ref{thm:hardnesscyclepath}).
We state our results on Paired Pattern Detection in Section \ref{sec:paired} by first showing hardness for Subset Pattern Detection (Theorem \ref{thm:set-hardness}) and then we state our algorithmic results. In section \ref{sec:c4lb} we state our lower bound for induced four cycle detection from $3$-Uniform $4$-Hyperclique Hypothesis.

\section{Preliminaries} \mina{depending on the number of pages, swap this with techniques section}
\label{sec:prelim}
For an integer $k$, let $P_k,C_k,K_k$ and $I_k$ be the path, cycle, clique and independent set on $k$ nodes.

Let $G$ be a graph and $S\subseteq V(G)$ be a subgraph of it. For every node $v\in V(G)$, define $N_S(v)$ to be the neighbors of $v$ in $S$. Define $d_S(v)=|N_S(v)|$.

A $k$-partite graph $G$ can be decomposed into $k$ partitions $G_1,\ldots,G_k$ where each $G_i$ is an independent set. For a pattern $H$ of size $k$ with vertices $v_1,\ldots,v_k$, we say that a graph $G$ is $H$-partite if it is a $k$-partite graph with $G_1,\ldots,G_k$ as its partitions such that there is no edge between $G_i$ and $G_j$ if $v_iv_j$ is not an edge in $H$. 

Let $G$ be an $H$-partite subgraph for a pattern $H$. We say that subgraph $H'$ of $G$ is a \textit{colorful} copy of $H$ if $H'$ has exactly one node in each partition of $G$. Note that if the vertices of $H'$ are $u_1,\ldots,u_k$ where $u_i$ is a copy of $v_i$ for all $i$, then $u_i$ must be in $G_i$ for all $i$. This is because for every $i,j$ where $v_iv_j$ is an edge, there must be an edge between the vertex of $H'$ that is in $G_i$ and the vertex of $H'$ that is in $G_j$. Otherwise, the number of edges of $H'$ is going to be smaller than the number of edges of $H$. 

For a set of patterns $S$, by (induced) \textit{$S$-detection} we mean finding a (induced) copy of one of the patterns in $S$, or indicating that there is no copy of any of the patterns in $S$.

Let $f:\{1,\ldots,c\}\rightarrow V(H)$ be a \textit{proper} coloring of the graph $H$ if the color of any two adjacent nodes is different. Let the \textit{chromatic number} of a graph $H$ be the smallest number $c$ such that there exists a proper coloring of $H$ with $c$ colors. We say that a graph $H$ is \textit{color critical} if the chromatic number of $H$ decreases if we remove any of its nodes. 

We call the subgraph $C$ of a graph $H$ a {\em core} of $H$ if there is a homomorphism $H\rightarrow C$ but there is no homomorphism $H\rightarrow C'$ for any proper subgraph $C'$ of $C$. Recall that a graph which is its own core is called simply a {\em core}. Moreover, any graph has a unique core up to isomorphisms, and the core of a graph is an {\em induced} subgraph of it \cite{hell1992core}.



\section{Technical Overview}\label{sec:technical-overview}\mina{removed algorithmic results overview, and hyperclique overview}
%We start this section with our algorithmic results in paired pattern detection. Each algorithm is quite technical (which is maybe not surprising given the algorithm of \cite{4path} for detecting induced $P_4$), and each has its own techniques. However, there are some similarities between the algorithms.
%For instance, when we develop our algorithms for detecting $\{H,\bar{H}\}$ for $4$-node patterns $H$, we start by running the known algorithm for detecting $\{I_4,K_4\}$ of Boppana and Halld{\'{o}}rsson~\cite{BoppanaH92} and finding a maximal clique or independent set.
%Then we try to find an $H$ or $\bar{H}$ that intersects with the maximal clique (or independent set) and finally if we find no such pattern, we prove the graph has a specific structure. 
%Merging all these algorithms in one simple algorithm is an interesting open problem. 

%Now we focus on the lower bound results. For our lower bound for induced $4$-cycle detection under $3$-uniform $4$-hyperclique hypothesis we start from a $3$-uniform hypergraph $G$ with $4$ partitions $V_1,V_2,V_3$ and $V_4$ and we want to find a $3$-uniform $4$-hyperclique in $G$ with one vertex in each partition. The reduction graph has the following $4$ partitions: $V_i\times V_{i+1}$ for each $i$, indices taken mod $4$. We put edges between $V_i\times V_{i+1}$ and $V_{i+1}\times V_{i+2}$ to encode the hyperedges in $G$, and we put edges inside each partition to enforce any induced $4$-cycle to have exactly one node in each partition. Note that this is the first reduction that only works for induced $H$ detection for a pattern $H$, and hence it might be a step forward to separate induced and non-induced $H$ detection, especially in the case of $H$ being the $4$-cycle.
%** the reduction from hyperclique \mina{Virginia: can you mayber write a few sentences about this?}
Here we give high level overview of our techniques. 
To understand our lower bounds for $k$-node patterns, we should first give an overview of the techniques used in \cite{stoc-paper}. In their first result \cite{stoc-paper} shows that if $H$ is $t$-chromatic and has a $t$-clique, then it is at least as hard to detect as a $t$-clique.
\paragraph{Reduction (1) \cite{stoc-paper}.} To prove the result of \cite{stoc-paper}, suppose that we want to reduce detecting a $t$-clique in a host graph $G=(V,E)$ to detecting $H$ in a graph $G^*$ built from $G$ and $H$. We build $G^*$ by making a copy $G^*_h$ of the vertices of $G$ for each node $h\in H$ as an independent set. Then if $hh'\in E(H)$, we put edges between $G^*_h$ and $G^*_{h'}$ using $E$: if $uw\in E$, then we connect the copy of $u$ in $G^*_h$ to the copy of $w$ in $G^*_{h'}$. Note that we have edges between $G^*_h$ and $G^*_{h'}$ if and only if $hh'$ is an edge and this enforces an encoding of $H$ in $G^*$ (we refer to $G^*$ as being $H$-partite).

To show that this reduction works, first suppose that there is a $t$-clique $\{v_1,\ldots,v_t\}$ in $G$. To prove that there is a $H$ in $G^*$, we consider a $t$ coloring of the vertices of $H$, and then we pick a copy of $v_i$ from $G^*_h$ if $h$ has color $i$. Using  the structure of $G^*$ and the fact that no two adjacent nodes in $H$ have the same color, one can show these $|H|$ nodes form a copy of $H$. For the other direction, suppose that there is a copy of $H$ inside $G^*$. This copy contains a $t$-clique $\{w_1,\ldots,w_t\}$. Since each $G^*_h$ is an independent set, no two nodes of the $t$-clique are in the same $G^*_h$. Moreover, the edges in $G^*$ mimic the edges in $G$ and this is sufficient to conclude that no two nodes of the $t$-clique are copies of the same node in $G$, and the original nodes in $G$ that the nodes $w_i$ are the copies of, form a $t$-clique. See Figure \ref{fig:reduction1}.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{reduction1.pdf}
    \caption{Reduction (1) construction: Reducing $K_3$-detection in $G$ to $H$-detection in $G^*$ for $H$ being the Diamond. The pattern $H$ is $3$ colorable and has a $3$-clique.}
    \label{fig:reduction1}
\end{figure}



Now we show how we modify this reduction to prove our first result, Theorem \ref{thm:psihardness}.
\paragraph{Reduction (2).}
We prove that if the size of the largest clique minor of a pattern $H$ is $\mu(H)$, then detecting a $\mu(H)$-clique in a graph $G$ can be reduced to detecting a colorful copy of $H$ in a graph $G^*$ that is constructed from $G$ and $H$ (Theorem \ref{thm:psihardness}). Reduction (1) above is good at catching cliques that are in the pattern $H$, but $H$ might not have a clique of size $\mu(H)$ in it, so we need a way to encode the clique minor of $H$ in $G^*$ so that it translates to a clique in $G$. To do that, we use a second method to put edges between $G^*_h$ and $G^*_{h'}$ when $hh'$ is an edge. We consider a clique minor of $H$ of size $\mu(H)$. Note that the clique minor partitions the vertices of $H$ into connected subgraphs with at least one edge between every two partition. Now if $hh'$ is an edge in $H$ and $h$ and $h'$ are in the same partition in the clique minor, we want to treat them as one node. So we put a ``matching" between $G^*_h$ and $G^*_{h'}$: for any node $v\in V(G)$, we put an edge between the copy of $v$ in $G^*_h$ and the copy of $v$ in $G^*_{h'}$. This way we show that whenever there is a colorful copy of $H$ in $G^*$, if $h$ and $h'$ are in the same partition of the clique minor of $H$, the vertices that are selected from $G^*_h$ and $G^*_{h'}$ must be copies of the same node in $G$. This means that each clique minor partition of $H$ represents one node in $G$. For $h$ and $h'$ that are not in the same clique minor partition, we put edges between $G^*_h$ and $G^*_{h'}$ the same as Reduction (1) (mimicking $E$). Using the rest of the properties of the construction, we show that the set of nodes that each clique minor partition represents are all distinct, and they form a $\mu(H)$-clique in $G$. 

Note that \cite{stoc-paper} uses the idea in Reduction 2 (a second method to define the edges of $G^*$) in a separate result. However the use of clique minors in \cite{stoc-paper} is indirect; it is coupled with the chromatic number and proper colorings of $H$, and in our results we directly use clique minors without using any other properties, thus avoiding the Hadwiger conjecture. 

%The proof of Theorem \ref{thm:psihardness} has the construction of a result of \cite{stoc-paper} as its base. This result states that if $H$ is $t$-chromatic and has a $t$-clique, then it is at least as hard to detect as a $t$-clique. The technique used in the reduction of \cite{stoc-paper} is as follows: Suppose we want to reduce detecting a $t$-clique in a host graph $G$ to detecting $H$ in a graph $G^*$ built from $G$. The reduction graph $G^*$ is an $H$-partite graph, where each partition is a copy of $G$. In the result of \cite{stoc-paper} either two partitions have no edges between them, or the edges between two partitions is the same as the edges between $G$, i.e. if $u$ and $v$ are attached in $G$, then $u$ in one partition is attached to $v$ in the other partition in $G^*$. 
%To make this reduction work for Theorem \ref{thm:psihardness}, we use a third type of edge set between partitions of $G^*$ (also used in a separate result of \cite{stoc-paper}), which adds a complete matching between two partitions. We further use a coloring on $H$ which ``imposes" a $t$-clique minor on $H$, and using this coloring we determine which type of edge set we need between each partition in $G^*$. Note that the use of clique minors in \cite{stoc-paper} is indirect; it is coupled with the chromatic number and proper colorings of $H$, and in our results we directly use clique minors without using any other properties. 
%\virgi{Maybe we should say that something is new? It is a new theorem right? It also talks about minors, not chromatic number...}

Another thing to note about Reduction (2) is that we are reducing a clique detection problem to a ``partitioned" subgraph isomorphism (PSI) problem. The reduction immediately fails if one removes the partitioned constraint. The reason is that we no longer can assume that if the reduction graph $G^*$ has a copy of $H$, then the nodes are in different vertex subsets $G^*_h$. If $G^*$ has a copy of $H$ and two nodes $v,u$ of this copy are in one vertex subset $G^*_h$, then we don't know if $v$ and $u$ are adjacent in $G$ or not. This can get in the way of finding a clique of the needed size in $G$. So if we want to get any result stronger than Reduction (1) for SI (and not PSI), we need to add new ideas. We introduce some of these new ideas below.

\paragraph{Reduction (3): paths and cycles.}
In Theorem \ref{thm:hardnesscyclepath} we show that if $H$ is the complement of a cycle or a path, then we can reduce detecting a $(\mu(H)-2)$-clique in a graph $G$ to detecting a copy of $H$ in a graph $G^*$ constructed from $G$ and $H$. 

As mentioned above, removing the partitioned constraint from reduction (2) doesn't directly work. However, when the graph is a core, it does work, and that is because PSI and SI are equivalent for cores \cite{marx2007can}. 
%We add new ideas to the construction of Theorem~\ref{thm:psihardness} to get stronger hardness results for paths and cycles and we believe that these ideas should be applicable to other pattern classes. 
%The reason that the approach of Theorem \ref{thm:psihardness} doesn't directly work for a pattern $H$ that is not a core is the following. In this approach we reduce finding a $t$-clique in a host graph $G$ to finding $H$ in an $H$-partite reduction graph $G^*$ with $t$ being the size of the maximum clique minor of $H$. 
When $H$ is a core, there is only one homomorphism from $H$ to itself, which means that there is only one type of ``embedding" of $H$ in the reduction graph $G^*$, and it is the embedding with exactly one vertex in each vertex subset $G^*_h$ of $G^*$. However, when $H$ is not a core, there can be multiple embeddings of $H$ in $G^*$, and these embeddings do not necessarily result in finding a copy of a $t$-clique in $H$, for $t\approx \mu(H)$.

In order to solve this issue of multiple embeddings, we ``shrink" some of the vertex subsets ($G^*_h$s) of the reduction graph $G^*$. More formally, we replace some of these subsets in $G^*$ by a single vertex. We do it in such a way that the only embedding of $H$ in $G^*$ is the one with exactly one vertex in each subset. This way, the rest of the argument of Reduction (2) goes through. There is a cost to shrinking these subsets: shrinking more subsets results in reducing the size of the clique that we reduce from. So the harder part of this idea is to carefully decide which partitions to shrink, so that we only lose a small constant in the size of the clique detection problem that we are reducing from. 

Recall that in Reduction (2) we consider a $\mu(H)$ clique minor of $H$ which partitions the vertex set of $H$ into $\mu(H)$ connected subgraphs. Here we observe that for $H$ that is the complement of a path or a cycle, we can select two particular partitions of the clique minor, and shrink vertex subsets $G^*_h$ for vertices $h$ that belong to one of these two partitions. This way we eliminate all the unwanted embeddings of the pattern $H$ in $G^*$, and reduce $(\mu(H)-2)$-clique detection in $G$ to $H$ detection in $G^*$. We note that the techniques in Reduction (3)  are of independent interest and can be potentially used for other graph classes.

%We observe that shrinking the vertex sets associated to only two partitions
%In Reduction (2) we use a $t$-coloring that defines a $t$-clique minor on the pattern and this coloring carries over to the partitions of the reduction graph $G^*$. For paths and cycles, we  shrink partitions associated to two colors, and hence we are effectively reducing $(t-2)$-clique detection to $H$-detection instead of $t$-clique, for $t$ being the size of the maximum clique minor of the pattern. These partitions are selected carefully, so that we can remove all the unwanted embeddings of our pattern in $G^*$. 


%\mina{Reviewer wants this: a short description of why a nThis would make it easier to appreciate the solution via a minimum size C-covering. atural first attempt (producing the "natural" reduction graph for every copy of C in H) does not work out. }
We now move on to our next reduction.
\paragraph{Reduction (4).}
Our next main result is Theorem \ref{thm:general-hardness}, which states that if $C$ is the core of the pattern $H$, then detecting $C$ in a graph $G=(V,H)$ can be reduced to detecting $H$ in a graph $G^*$ which is constructed from $G$ and $H$.

First note that Reduction (1) doesn't directly work here. This is because if $G$ has a copy of $C$, we have no immediate way of finding a copy of $H$ in $G^*$. Recall that in Reduction (1) we used a coloring property of $H$ to do this.

As a first attempt to such a reduction, one might use the following idea of Floderus et al. \cite{FloderusKLL15}. They showed that any pattern that has a $t$-clique that is disjoint from all the other $t$-cliques in the pattern is at least as hard as $t$-clique to detect. 
Here we explain their idea in the context of reducing $core(H)$-detection to $H$ detection. Let $C'$ be a copy of $C$ in $H$. The idea is to build the reduction graph of Reduction (1) using $C'$ as the pattern, and to add the rest of the pattern $H$ to it.
More formally, 
for any node $h$ in $C'$, let $G^*_h$ be a copy of $V$, the set of vertices of $G$. Put edges between $G^*_h$ and $G^*_{h'}$ same as before if $hh'$ is an edge. Call this graph $G^*_{C'}$. To complete the construction of $G^*$, add a copy of the subgraph $H\setminus C'$ to $G^*_{C'}$, and connect a vertex $h'$ in this copy to all the nodes in $G^*_h$ for $h\in C'$ if $hh'$ is an edge in $H$. 

The reason we construct the Reduction (1) graph on $C'$ is that if $G$ has a copy of $C$, then we can find a copy of $C$ in $G^*_{C'}$ using the arguments in Reduction (1). This copy of $C$ and all the vertices in $G^*\setminus G^*_{C'}=H\setminus C'$ form a copy of $H$. For the other direction, suppose that there is a copy $H^*$ of $H$ in $G^*$. We hope that this copy contains a subgraph $C''$ that is completely inside $G^*_{C'}$, so that then this leads us to a copy of $C$ in $G$ using the properties of $G^*_{C'}$ and the fact that $C$ is a core. However, such a construction cannot guarantee this, and in fact there might be no copies of $C$ in $H^*$ that are completely in $G^*_{C'}$.  %For any $h$ outside this copy, just put a copy of the vertex $h$. We put edges between $V_h$ and $V_{h'}$ same as before, 

So we need to find a subgraph $H'$ of $H$, so that if we build the reduction graph $G^*_{H'}$ of Reduction (1) on it, it has the property that if $G $ has a copy of $C$, then we can find a copy of $H'$ in $G^*_{H'}$. 

To do this, we simplify and use an idea of \cite{stoc-paper}. In particular, \cite{stoc-paper} introduces the notion of $(K_t,F)$-minor colorability of a pattern $B$, which is a coloring of $B$ with $t$ colors such that the coloring imposes a $t$-clique minor on any copy of $F$ in $B$. Then using this definition, one finds a minimal covering of the graph $H$ with $(K_t,F)$-minor colorable subsets and one argues that one can take one of these subsets as $H'$.% consider one of these subsets, build the Reduction (1) construction on it, and add the remainder of the pattern to it. 

We notice that the properties that \cite{stoc-paper} uses relating the chromatic number and the clique minor of a pattern in this construction can be summarized into the core of patterns. We introduce the notion of $F$-coloring, which simply says that if $B$ is $F$-colorable then there is a coloring such that any copy of $F$ in $B$ is a colorful copy under this coloring. Then we cover $H$ with minimal number of $C$-colorable subsets. We show that we can take one of these subsets as $H'$.
%Note that the minor part of the $(K_t,F)$-minor colorability is not needed since it is captured when $F$ is a core. 

%The proof of this theorem uses similar techniques as the main result of \cite{stoc-paper}. Indeed, we use a similar framework, but we notice that the properties that \cite{stoc-paper} uses relating the chromatic number and the clique minor of a pattern can be summarized into the core of patterns without using the chromatic number or clique minor of the pattern. This helps us simplify some of the notions. For example \cite{stoc-paper} has the notion of $(K_t,F)$-minor colorability of a pattern $H$, which is a coloring of $H$ with $t$ colors such that the coloring imposes a $K_t$ minor on any copy of $F$. In comparison, we have the notion of $F$-coloring, which simply says that any copy of $F$ is a colorful copy under this coloring. The minor part of the $(K_t,F)$-minor colorability is not needed since it is captured when $F$ is a core. 

 %The next lemma helps us characterize automorphisms of paths and cycles, and so it helps us find the appropriate partitions of $G^*$ to shrink.

%We show that we can change this construction for patterns $H$ that are not core so that the theorem works for them as well. Our idea is to simply ``shrink" some of the partitions of $G^*$ to only include one node. The hard part is to do this to as few partitions as possible. We show that in the case of paths and cycles, we can need to only shrink two partitions, and this helps us limit the way the pattern $H$ can be ``embedded" in $G^*$.

%\mina{make sure we don't explain these things again too much in the text.}

%\mina{talk about our techniques: for lower bounds, we generalize the stoc paper. For paths and cycles, we use newer techniques which might be useful for other potential lower bounds.}


%\mina{ say the difference and similarities between this paper and the stoc paper?}\virgi{in a special technical overview section?}

%\virgi{This should be in some technical overview section.}
%\mina{similarities to the stoc paper: we have the following notions in the stoc paper: $(K_t,F)$-minor colorability of a graph $H$: a coloring of $H$ with $t$ colors, such that it imposes a $K_t$ minor on any copy of $F$, meaning that if you consider a copy of $F$, each color is one component of the $K_t$ minor. Also $F$ should be $t$-chromatic.\\ $F$-covering of graph $H$: if $t$ is the chromatic number of $F$, then we want to cover all the copies of $F$ in $H$ with $(K_t,F)$-minor colorable subgraphs.
%\\Here we have $F$-coloring: simply says that any copy of $F$ is colorful under this coloring.\\ 
%$F$-covering: cover all the subgraphs $F$ of a graph $H$ by $F$-colorable subgraphs.
%\\So the $F$-covering notions are the same except that the underlying coloring definition is different. Our definition is simpler, we use the properties of cores, wheras in the stoc paper hadwiger conjecture properties are used. Our version is more similar to the "clique covering" version of the stoc paper.
%}

Finally, we generalize Theorem \ref{thm:general-hardness} to the problem of detecting a pattern from a set $S$ of patterns in Theorem \ref{thm:set-hardness}. We show that if $S$ is a set of patterns, there is a pattern $H\in S$, such that detecting the core of $H$, $C$, in a graph $G$ can be reduced to detecting any pattern from $S$ in a graph $G^*$ constructed from $G$ and $S$. In fact, $G^*$ is the reduction graph of Reduction (4) on $H$ as the pattern. The main part of Theorem \ref{thm:set-hardness} is to find the appropriate $H$ in $S$. In order to find this pattern $H$, we look at homomorphisms between the patterns in $S$. In particular, we form a graph with nodes representing patterns in $S$ and directed edges representing homomorphisms. We look at a strongly connected component of this graph that has no edges from other components to it, so there is no homomorphism from any pattern outside this component to any pattern inside the component. We show that all the patterns in this component have the same core and we show that the pattern $H$ can be any of the patterns in this component.


% \subsection{Related work}
% Marx \cite{marx2007can} in his seminal paper ``Can you beat treewidth?" showed that if Subgraph Isomorphism can be solved in time $f(k)n^{o(k/logk)}$, where $f$ is an arbitrary function and $k = |E(H)|$ is the number of edges of the smaller graph $H$, then ETH fails. 

% Manurangsi, Rubinstein and Schramm~\cite{ManurangsiRS21} introduced the ``Strongish Planted Clique Hypothesis'', and showed that under this hypothesis for every $k$-node pattern $H$, there is no algorithm that solves the induced pattern detection problem on $n$-vertex graphs in time $f(k)\cdot n^{o(k)}$ for any function $f$.

% Bringmann and Slusallek \cite{bringmann2021current} showed that under the $3$-uniform hyperclique conjecture, for any $t\ge 3$, there exists a pattern $H$ with treewidth $t$ such that  Subgraph Isomorphism on pattern $H$ has no algorithm running in time $O(n^{t+1-\epsilon})$ for any $\epsilon>0$. This is in contrast to the algorithm of Alon, Yuster and Zwick \cite{alon1995color} for SI detection for patterns with treewidth $t$ in time $O(n^{t+1})$.

% Note that the results of Marx~\cite{marx2007can} and Bringmann and Slusallek~\cite{bringmann2021current} show hardness for specific classes of patterns, whereas the the results of Dalirrooyfard et al.~\cite{stoc-paper}, Manurangsi et al.~\cite{ManurangsiRS21} and this paper aim to determine hardness for \emph{any} $k$-node pattern.
%\mina{this result and Marx lower bound work for some classes of patterns wheras our lower bounds explain hardness for every single pattern.}







==> oldintrostuff.tex <==
--------------


\mina{old stuff below.}

% There are two versions of SI: {\em induced} and not necessarily induced, {\em non-induced} for short. In the induced version, the copy of $H$ in $G$ must have both edges and non-edges preserved, whereas in the non-induced version only edges need to carry over, and the copy of $H$ in $G$ can be an arbitrary supergraph of $H$.

% It is well known that the induced version of $H$-pattern detection for any $H$ of constant size is at least as hard as the non-induced version: there is a simple reduction from the non-induced version to the induced version using color-coding (see e.g. \cite{stoc-paper}).
% % Both notions require that there is a 1-to-1 mapping $\phi$ from the vertices of $H$ to the vertices of $G$ with special properties.

% % We say that $H$ is an induced subgraph of $G$ if the mapping $\phi$ is such that $(u,v)$ is an edge of $H$ if and only if $(\phi(u),\phi(v))$ is an edge of $G$. In contrast, $H$ is a non-induced subgraph of $G$ as long as whenever $(u,v)$ is an edge of $H$, then $(\phi(u),\phi(v))$ is an edge of $G$, but the non-edges of $H$ could be represented by edges of $G$.

% % When the number of nodes $k$ of $H$ is constant, it is not hard to reduce in linear time the non-induced version of SI of $H$ and an $n$-node $G$ to the induced version, for the same pattern $H$, but a different $G'$ on $O(n)$ nodes (say, via color-coding). Hence, the induced version of the problem is provably harder.

% % Additionally, SI for any $k$-node $H$ and $n$-node $G$ can be reduced in $O(n^2)$ time to detecting a $k$-clique in an $O(n)$ node graph, thus $k$-clique is the hardest pattern.

% % The fastest algorithms for $k$-clique
% %  procede via a reduction by Ne\v{s}etril and Poljak \cite{nevsetvril1985complexity} to $3$-clique which can then be solved using fast matrix multiplication \cite{Clique1}. For $k$ divisible by $3$, this results in a running time of $O(n^{\omega k/3})$, where $\omega<2.37286$ \cite{almanv21} is the exponent of square matrix multiplication. When $k$ is not divisible by $3$, the best known algorithm for $k$-clique runs in $C(n,k):=O(n^{\omega(\lfloor k/3\rfloor,\lceil k/3\rceil,\lceil (k-1)/3\rceil)})$ time via a generalization of the \cite{Clique1} reduction; here $\omega(a,b,c)$ is the exponent of multiplying an $n^a\times n^b$ by an $n^b\times n^c$ matrix.
 
% The $k$-clique running time $C(n,k)$ is the fastest known running time for many other $k$-node patterns.
% Nevertheless, some patterns are easier to detect than $k$-clique. This is especially true in the non-induced case (e.g. \cite{alon1995color,KowalukLL13}). For instance, $k$-paths, $k$-cycles, and more generally patterns of bounded treewidth can be found in $2^{O(k)}\textrm{poly}(n)$ time via the color-coding method~\cite{alon1995color}, where the exponent of the polynomial in $n$ depends on the treewidth but not on $k$. 

% In the induced case, many patterns are also easier than $k$-clique, e.g. for $k=3,4,5,6$, any $H$ that is not the $k$-independent Set or the $k$-clique can be found in the current best running time for $(k-1)$-clique \cite{williams2014finding,stoc-paper}. For $k\geq 7$, it is not known if all patterns other than $k$-clique and $k$-independent set can be solved faster than $k$-clique. This is however known to be true for ``combinatorial algorithms'' that avoid the impracticalities of algebraic matrix multiplicatopn: Bl\"{a}ser et al.~\cite{BlaserKS18} showed that all such patterns can be detected in $O(n^{k-1})$ time, whereas the best known ``combinatorial'' algorithms for $k$-clique run in $n^{k-o(1)}$ time.

% An intriguing question is: 
% \begin{center}{\em What makes some patterns easier to detect than others}?\end{center}

Prior work (e.g. \cite{stoc-paper,FloderusKLL15}) has largely approached this by giving reductions from $t$-clique to $H$ pattern detection, for $k$-node patterns $H$ and $t<k$. For a pattern graph $H$, we say that (induced/non-induced) $H$ is at least as hard as $t$-clique if there is an efficient reduction from $t$-clique in an $n$-node graph to $H$-detection in an $O(f(k) n)$-node graph for some function $f$ of $k$. Here the reduction is efficient if it runs in $C(n,t)^{1-\eps}$ time for some $\eps>0$, though typically the reductions run even faster, in $O(n^2)$ time.

If $H$ is at least as hard as $t$-clique,
then besides $H$ being so hard that it encodes the hardest $t$-node pattern, we also get some more quantative limitations on the running time for $H$ detection under popular hypotheses.
For instance, under the Exponential Time Hypothesis (ETH) \cite{ip01} detecting $H$ as a subgraph cannot be done in $n^{o(t)}$ time. Another popular hardness hypothesis is the $t$-clique Hypothesis that stipulates that $C(n,t)$ is the best possible running time for $t$-clique, up to $n^{o(1)}$ factors, in the word-RAM model of computation with $O(\log n)$ bit words (see e.g. \cite{vsurvey}). Under this hypothesis, if $H$ is at least as hard as $t$-clique, then $H$ also cannot be solved polynomially faster than $C(n,t)$ time. Moreover, if one focuses on ``combinatorial'' algorithms that avoid the Strassen-like matrix multiplication techniques, then any $H$ that is at least as hard as $t$-clique does not admit an $O(n^{t-\eps})$ time algorithm for $\eps>0$, unless $t$-clique does, and this is hypothesized to be impossible (e.g. \cite{vsurvey}).

Dalirrooyfard, Vuong and Vassilevska W.~\cite{stoc-paper} showed that for any $H$ that contains a $t$-clique, non-induced $H$ is at least as hard as $t$-clique. They also showed that, assuming the Hadwiger conjecture~\cite{hadwiger}, if $H$ has chromatic number $c$, then non-induced $H$ is at least as hard as $c$-clique. This in turn implied that under the Hadwiger conjecture, any $k$-node induced $H$ is at least as hard as $\sqrt k$-clique.
So far it has been open whether one needs to condition on the Hadwiger conjecture.


% In this paper we strengthen the hardness results of \cite{stoc-paper}, showing how to remove the dependence on the Hadwiger conjecture with a slight loss in the hardness, and also giving higher clique-based lower bounds for some patterns. We also introduce a variant of SI called Paired Pattern Detection that lies between the induced and non-induced variants. We develop nontrivial algorithms for this variant.



%**in related work: cite the rubinstein paper with a different hypothesis.


% **********

% Subgraph isomorphism is one of the most widely studied problems.

% induced/not induced

% algorithms for induced -- just clique
% for non-induced better

% etc.
% This work considers two questions
% - hardness
% - small pattern detection and extensions to ramsey ?

% (1)
% Hardness results:
% clique is the hardest pattern.
% how do other patterns relate to clique?

% prior work: 
% (1) every H containing a t-clique is at least as hard as t-clique even in the non-induced case (our stoc paper)
% (2) if H has chromatic number $t$, then under the Hadwiger conjecture, it's as hard as $t$-clique, even in the non-induced case.
% (3) as a corollary, under the Hadwiger conjecture, induced H is at least as hard as $\sqrt k$ clique.

% -- we show that if H has a clique minor of size $t$ then


% we improve this

% These imply hardness under ETH, and under the clique hypothesis?

\subsection{Our results}
In this paper we strengthen the hardness results of \cite{stoc-paper}, showing how to remove the dependence on the Hadwiger conjecture with a slight loss in the hardness, and also giving higher clique-based lower bounds for some patterns such as paths and cycles. We also introduce a variant of SI called Paired Pattern Detection that lies between the induced and non-induced variants. We develop nontrivial algorithms for this variant.


% \paragraph{Paired Subgraph Isomorphism.}
%  In many cases the induced version of the SI problem is much harder than the non-induced version. The simplest example is independent set, when the non-induced version is trivial, whereas the induced version is the hardest pattern detection problem. 
% The non-induced version of SI asks for a given pattern $H$ and a host graph $G$, if some supergraph of $H$ is an induced subgraph of $G$. Thus, intuitively the reason why the non-induced version is easier is because there are more options of what subgraph one can return.

% We explore this power of allowing an algorithm to return one of a {\em set of possible patterns}. This version of SI has practical applications as well: in  the analysis of social networks for instance, one might be interested in finding some small dense pattern signifying, for instance, a cluster of connected entities, but which dense pattern it is, it might not matter too much.

% In graph theoretical applications related to graph coloring, one is often concerned with $\{H,F\}$-free graphs for various patterns $H$ and $F$ (e.g. \cite{KarthickM18,DabrowskiP18,DabrowskiDP17}). Recognizing such graphs is thus of interest there as well. 

% The main question we are interested in addressing is, given two patterns $H$ and $F$, when is it easier to detect either an $H$ or an $F$, than detecting each individual one of $H$ or $F$ separately?

% We begin with the case of paired $3$-node patterns. We show that the Paired Pattern Detection problem is in $O(n^2)$ time for every pair of $3$ node patterns and any $n$ node host graph. Moreover, for all but two pairs of patterns, it is actually in linear time.

% We then focus on pairs of $4$ node patterns. Similarly to the $k=3$ case, we show that Paired Pattern Detection for any pair of $4$-node patterns is solvable faster than finding $4$-cliques. In particular, $4$-node Paired Pattern Detection is in $\tilde{O}(n^\omega)$ time where $\omega<2.37286$ \cite{almanv} is the exponent of matrix multiplication, whereas the fastest known algorithm for $4$-clique runs in supercubic, $O(n^{\omega(1,2,1)})$ time where $\omega(1,2,1)\leq 3.252$ \cite{legallurr} is the exponent of multiplying an $n\times n^2$ by an $n^2\times n$ matrix.

% An interesting question is then, for what pairs can we solve $4$-node Paired Pattern Detection faster than matrix multiplication time?

% We give the following general hardness result
% -->Theorem 
% \begin{theorem} Let $S$ is a set of patterns such that every $H\in S$ contains a $k$-clique. Then detecting whether a given graph contains some pattern in $S$ is at least as hard as $k$-clique.
% \end{theorem}

% The theorem is a consequence of a more general theorem that we prove 

% % -> in applications we might be happy with one of a small set of patterns. in theory recognizing $\{H,F\}$-free graphs is important (give citations); finally non-induced says that we are happy to find any supergraph of $H$, whereas induced only wants $H$. A scenario between induced and non-induced is having a set of admissible patterns.

% Here we study the case of $4$-node graphs. 
% A Ramsey result that follows from Erdos-Szekeres (cite Erdős, Paul; Szekeres, George (1935), "A combinatorial problem in geometry", Compositio Mathematica, 2: 463–470,) and Boppana, Halldorsson (cite APPROXIMATING MAXIMUM  INDEPENDENT SETS BY EXCLUDING SUBGRAPHS) shows that in linear time one can find either a log size independent set or a log size clique in any graph. This motivates us to ask if for any $H$ there is a fast algorithm that either finds $H$ or its complement (or decides neither exists).

% Indeed, we should that for $4$ node patterns $H$ there is an $O(n^2)$ time algorithm that does this.

% We know that finding any $4$-node pattern containing a triangle is at least as hard as triangle detection, so it needs at least $n^\omega$ time, where currently the best bound on $\omega$ is $2.372...>7/3$.
% Another pattern that has been studied a lot (cite) is the induced $4$-cycle; the fastest algorithm is also $n^\omega$, but no lower bounds are known. non-induced $4$-cycle is easier, solvable in $O(n^2)$ time (cite). Unknown why the induced case is harder. Known reduction techniques from clique fail. + Mina's two arguments on why interesting

% If $C_4$ is at least as hard as triangle, one might expect that finding at least one of 4-clique and $C_4$ would still need triangle detection time (this is only intuition, not a formal statement). However, we show that for any $H$, finding one of $H$ or $C_4$ can be done in $O(n^{7/3})$ time. For some $H$, the running time is even faster.

% This might be some indication that $C_4$ could be easier than triangle detection?


% **********

% pattern set motivation: (1) in coloring they care a lot about induced $\{H,F\}$ free graphs for small subgraphs $H,F$. (2) something between induced and non-induced.

% say about psi, stoc paper, the strongish clique conjecture paper.


% %Subgraph Isomorphism with two versions of it has been studied for a long time [some references] especially from an algorithm point of view. If the treewidth of a pattern $H$ is $tw(H)$, Alon, Yuster and Zwick \cite{alon1995color} gave an algorithm for detecting $H$ in an $n$-node graph $G$ in time $O(n^{tw(H)+1})$. For the induced version of the problem,
% %a standard generalization of a result of Ne\v{s}etril and Poljak \cite{nevsetvril1985complexity} shows that any $k$-node pattern can be detected in $O(n^{kw/3})$ time in an $n$-node graph as an induced subgraph. This running time is conjectured to be optimal for detecting $k$-clique, and is regarded as the ``$k$-clique conjecture". For small values of $k$ there has been better algorithms for patterns that are not cliques or independent sets \cite{blaser2018graph,williams2014finding}.

% %On the lower bound side of the problem, Marx \cite{marx2007can} showed that if partitioned subgraph isomorphism (PSI) in $n$-node graphs can be solved in $f(m)n^{o(m/\log{m})}$ time where $f$ is some function and $m$ is the number of the edges of the pattern, then ETH fails. Let \textit{core} be a graph that has no homomorphism to a proper subgraph of itself (Examples of cores are complete graphs, odd cycles and color critical graphs). Then since PSI on core graphs is equivalent to subgraph isomorphism, \cite{marx2007can} concludes that if subgraph isomorphism in $n$-node graphs can be solved in $f(m)n^{o(m/\log{m})}$ time where $f$ is an arbitrary function and $m$ the number of edges of the pattern, then ETH fails.

% %The lower bound results of Marx \cite{marx2007can} are corollaries of a hardness result he gives on binary CSP.% Note that this result doesn't talk about the hardness of each particular pattern. 
%  %A more ``fine-grained" lower bound on subgraph isomorphism is given by \cite{stoc-paper}, where they prove that if a pattern $H$ has a clique of size $t$, then it is as hard to detect as a $t$-clique, giving a lower bound of $\Omega(n^{\log k})$ on the hardness of ``induced" detection of $k$-node patterns in $n$-node graphs. Moreover, they showed that under the Hadwiger Conjecture \cite{hadwiger}, if a pattern is $t$-chromatic, then it is at least as hard to detect as a $t$-clique, giving a lower bound of $\Omega(n^{\sqrt{k}})$ on the hardness of ``induced" detection of $k$-node patterns in $n$-node graphs under the Hadwiger Conjecture.
 
%\subsection{our results}


\paragraph{Stronger Conditional Lower Bounds.}
%\mina{these are written long time ago, it might be better to remove relating it to psi.}


%We first give a lower bound for the hardness of Partitioned subgraph isomorphism (PSI) which we show later that works for subgraph isomorphism for patterns that are "core", since subgraph isomorphism of cores is equivalent to partitioned subgraph isomorphism of them.

We call a subgraph $C$ of a graph $H$ a {\em core} of $H$ if there is a homomorphism $H\rightarrow C$ but there is no homomorphism $H\rightarrow C'$ for any proper subgraph $C'$ of $C$. A graph which is its own core is called simply a {\em core}.
Hell and Ne{\v{s}}et{\v{r}}il~\cite{hell1992core} showed that every graph has a unique core (up to isomorphism), and the core of a graph is an {\em induced} subgraph. We denote the core of a graph $H$ by $core(H)$. 
We prove strong hardness results for pattern graphs that are cores, relating the hardness of detecting the pattern to the size of its maximum clique minor. We then relate the hardness of detecting arbitrary patterns to the hardness of detecting their cores. Our approach is similar to that of Dalirrooyfard, Duong Vuong and Vassilevska W.~\cite{stoc-paper} who related the hardness of pattern detection to the size of the maximum clique or the chromatic number of the pattern.

We begin with a theorem that shows hardness for detecting a ``colorful'' copy of a pattern $H$. Here the vertex set of the host graph $G^*$ is partitioned into $k$ parts, and one is required to detect an induced copy of a $k$-node $H$ so that the image of the $i$th node of $H$ is in the $i$th part of the vertex set of $G^*$. This version of SI is often called Partitioned Subgraph Isomorphism (PSI).  Marx \cite{marx2007can} showed that under ETH, PSI for a pattern $H$ requires at least $n^{\Omega(tw(H)/\log{tw(H)})}$ time where $tw(H)$ is the treewidth of $H$. We give a more fine-grained lower bound for PSI. We give a reduction from $\eta$-clique detection in an $n$ node graph to PSI for a graph $H$ in an $O(n)$ node host graph, for any $H$ with maximum clique minor of size  $\eta$.%\virgi{Do you mean clique number or clique minor number?}

\begin{restatable}{theorem}{psihardness}
\label{thm:psihardness} 
\textbf{(Hardness of PSI)} Let $H$ be a $k$-node pattern with maximum clique minor of size $\eta(H)$, and let $G$ be an $n$-node graph. Then one can construct a $k$-partite $O(n)$-node graph $G^*$ in $O(n^2)$ time such that $G^*$ has a colorful copy of $H$ if and only if $G$ has a clique of size $\eta(H)$.
\end{restatable}




Thomason \cite{thomason2001extremal} gives an estimate on the size of the maximum clique minor of any graph as follows. Let $c(t)$ be the minimum number such that every graph $H$ with $|E(H)|\ge c(t)|V(H)|$ has a $K_t$ minor. Then $c(t)=(\alpha+o(1))t\sqrt{\log{t}}$, where $\alpha\le 0.32$ is an explicit constant. Since for $t=\frac{|E(H)|/|V(H)|}{\sqrt{\log (|E(H)|/|V(H)|)}}$ the above inequality is true, we have the following corollary. 
\begin{corollary}
Let $H$ be a $k$-node $m$-edge pattern. Then the problem of finding a colorful copy of $H$ in an $n$-node $k$-partite graph is at least as hard as finding a clique of size $\frac{m/k}{\sqrt{\log{m/k}}}$ in an $O(n)$-node graph.
\end{corollary}

Hence, for example if $m=ck^2$ for some constant $c$, then the PSI problem for $H$  cannot be solved in $n^{o\left({\frac{k}{\sqrt{\log{k}}}}\right)}$ time. Thus, for dense enough graphs, we 
improve the lower bound of $n^{\Omega(tw(H)/\log{tw(H)})}$ due to Marx \cite{marx2007can}, since $tw(H)\le k$.
% \mina{so we have $tw(H)=O(k)$ in this case: because $tw$ of any graph is at least the minimum degree of the graph, and so there is a subgraph $H'$ of $H$ having min degree $ck$, and since $tw(H)\ge tw(H')$, we have $tw(H)\ge ck$.}

% \mina{so for dense graphs, we improve the lower bound of Marx by $\sqrt{\log}$ in the exponent. Was he maybe asking if we can do that in his paper?}




%technique: The problem of having repeatedd vertices: color coding.
%\subsection{(Induced) subgraph isomorphism}
%Here we move to a generalization of the approach of \cite{stoc-paper} on giving lower bounds for SI. 
%The first hardness result on subgraph isomorphism with core patterns is by Marx \cite{marx2007can} where he showed that PSI and SI are equivalent on cores, and so using his PSI lower bound, by ETH detecting a core pattern $H$ in an $n$-node graph requires  $n^{\Omega{(tw(H)/\log{(tw(H)}))}}$ time where $tw(H)$ is the treewidth of $H$.  
%We give the first fine-grained hardness (correct term?) result on cores, using Theorem \ref{thm:psihardness}.
%From the equivalence of Subgraph Isomorphism and PSI on cores, we have the following hardness result on cores due to Theorem \ref{thm:psihardness}.


While Theorem~\ref{thm:psihardness} only applies to PSI, one can use it to obtain hardness for SI as well, as long as $H$ is a core. In particular, Marx~\cite{marx2007can} showed that PSI and SI are equivalent on cores. Thus we obtain:

\begin{restatable}{corollary}{corehardnessinsi}
\label{thm:core-hardness}
\textbf{(Hardness of cores in SI)} Let $G$ be an $n$-node $m$-edge graph and let $H$ be a $k$-node pattern with maximum clique minor of size $\eta(H)$. If $H$ is a core, then one can construct a graph $G^*$ with at most $nk$ vertices in $O(m+n)$ time such that $G^*$ has a subgraph isomorphic to $H$ if and only if $G$ has a $\eta(H)$-clique as a subgraph.
\end{restatable}


While Corollary~\ref{thm:core-hardness} only applies to cores, we are able to use it to show strong hardness for induced path and cycle detection, as we will discuss later. The statement of the corollary is similar in spirit to one of the results of \cite{stoc-paper} that related the hardness of a pattern to that of its chromatic number.

% \mina{We use this result for getting better bounds for paths and cycles, where we modify this construction using new ideas, and those ideas might be useful for other pattern in future works. This is the main motivation for this theorem.}


% \mina{This result is similar to the simple case of theorem 2.1 in the stoc paper. That result says that if $H$ is $t$-chromatic, you can reduce $t$-clique detection to $H$-detection.

Corollary~\ref{thm:core-hardness} applies to the non-induced version of SI. We obtain a stronger result for the induced version.

\begin{restatable}{corollary}{corehardnessgeneral}
\label{cor:coreLB}
\textbf{(Hardness for induced-SI for cores)}
Let $H$ be a $k$-node pattern which is a core. Suppose that $w(H)$ is the size of the maximum clique in $H$. Then detecting $H$ in an $n$-node graph as an induced subgraph is at least as hard as detecting a clique of size $\max\{\sqrt{(k+2w(H))/2},\sqrt{k/1.95}\}$.
\end{restatable}


For a comparison, the result of \cite{stoc-paper} shows that
 non-induced SI for any $k$-node $H$ is at least as hard as detecting a clique of size $\sqrt{k}$, but the result is conditioned on the Hadwiger conjecture. 
 Corollary \ref{cor:coreLB} is the strongest known clique-based lower bound result for $k$-node {\em core} $H$ that is not conditioned on the Hadwiger conjecture.

%Finally we improve this result for cycles of size $4t+1$ by a factor of $n^{0.5}$.

%Using the techniques in the proof of Theorem \ref{thm:core-hardness}, we conclude that induced-$C_k$ and induced-$P_k$ detection is at least as hard as $(\floor{\frac{3k}{4}}-2)$-clique detection, which improves the previous lower bound, saying that it is as hard as $k/2$-clique detection [stoc paper]. 

%To show hardness for general graphs, we define the notion of an "absolute core". $C$ is an absolute core of $H$ if there $C$ is a core graph and a subgraph of $H$ and if there is a homomorphism from $C$ to $C'$ which is a subgraph of $H$, then $C'$ and $C$ are isomorphic. 

Our next theorem relates the hardness of detecting a pattern to the hardness of detecting its core.

\begin{restatable}{theorem}{generalhardness}
\label{thm:general-hardness}
Let $G$ be an $n$-node $m$-edge graph and let $H$ be a $k$-node pattern. Let $C$ is the core of $H$. Then one can construct a graph $G^*$ with at most $nk$ vertices in $O(n^2)$ time such that $G^*$ has a subgraph isomorphic to $H$ if and only if $G$ has a subgraph isomorphic to $C$, with high probability\footnote{with probability $1/\poly{n}$}.
\end{restatable}


Given Theorem~\ref{thm:general-hardness}, we are able to show that under ETH, there can be no $n^{o(\sqrt{k}/\log{k})}$ time algorithm for detecting any $k$-node $H$ as an induced subgraph of an $n$ node host graph.

\begin{restatable}{corollary}{inducedsihardness} 
\label{cor:induced-si-hardness}
\textbf{(Hardness of Induced-SI)}
For any $k$-node pattern $H$, the problem of detecting an induced copy of $H$ in an $n$-node graph requires $n^{\Omega{(\sqrt{k}/\log{k})}}$ time under ETH. 
\end{restatable}

\mina{add $n^{k^{1/4}}$ lower bound from cor 1.3 as a result without eth.}

Recall that
\cite{stoc-paper} shows that induced-SI for any $k$-node $H$ is at least as hard as $\sqrt k$-clique, and hence under ETH, needs $n^{\Omega\left(\sqrt k\right)}$ time.
However that result is
 \textbf{conditioned on the Hadwiger conjecture}.
 The above corollary gives a slightly weaker lower bound \textbf{independent} of the Hadwiger conjecture. 
 

%\virgi{This should be in the text as a proof, not in the intro:}



%Note that the above lower bound is in terms of the size of the graph wheras the lower bound of Marx is in terms of the treewidth.



\paragraph{Hardness of paths and cycles.}
%\mina{maybe give some reasoning on why we focus on paths and cycles, for example maybe that paper that does ${P_s,C_t}$-free coloring}
Recognizing graphs with no induced cycles and no induced paths of certain length is of interest for instance in the area of graph coloring (e.g. \cite{GolovachPS14,HH17}). 
Floderus, Kowaluk, Lingas and Lundell~\cite{FloderusKLL15} (see also \cite{stoc-paper}) showed that both induced $(2k-1)$-Path and induced $2k$-Cycle are at least as hard as $k$-clique. Meanwhile, the fastest algorithms for induced $P_k$ and $C_k$ detection for general $k$ is the same as for $k$-clique detection. If one considers only combinatorial algorithms, then both induced $P_k$ and $C_k$ have $O(n^{k-2})$ time algorithms~\cite{BlaserKS18}, the running time of $(k-2)$-clique detection. This is far from the $\lceil k/2\rceil$-clique based lower bound of \cite{FloderusKLL15}.

Our goal is to obtain higher hardness for induced path and cycle detection, in order to explain the gap between the known algorithms and lower bounds.

A first attempt would be to use Theorem \ref{thm:general-hardness}. However, since paths and cycles of even length, or their complements are not cores and their core and their complement's core is no bigger than a $\ceil{k/2}$-clique, Theorem \ref{thm:general-hardness} only states that detecting a $k$-Cycle or $k$-Path is at least as hard as detecting a $\ceil{k/2}$-clique. This is no better than the result of \cite{FloderusKLL15}.

It turns out that Theorem \ref{thm:general-hardness} does apply for cycles of odd length. We prove that for odd $k$, the complement of $C_k$ is a core and has a maximum clique minor of size $\ceil{3k/4}$ for $k\equiv 1 \pmod{4}$ and $\floor{3k/4}$ for $k\equiv 3 \pmod{4}$.
Therefore, Corollary \ref{thm:core-hardness} states that detecting an odd length $C_k$ is at least as hard as detecting a clique of size $\ceil{3k/4}$ for $k\equiv 1 \pmod{4}$ and a clique of size $\floor{3k/4}$ for $k\equiv 3 \pmod{4}$.

The size of the maximum clique minor of the complements of all paths and cycles of size $k$ is roughly $3k/4$, up to floors and ceilings. However, 
we cannot directly get the same hardness bound as for odd $k$-cycles,
 for paths and even cycles. However, we develop a new technique, and are able to
 prove roughly the same bound for $k$-paths and even $k$-cycles, sacrificing only a constant in the exponent of the lower bound. More precisely, we show the following theorem which concludes that induced-$C_k$ and induced-$P_k$ detection are at least as hard as $(\floor{\frac{3k}{4}}-2)$-clique detection.
\begin{restatable}{theorem}{hardnesscyclepath}
\label{thm:hardnesscyclepath}
\textbf{(Hardness of $P_k$ and $C_k$)}
Let $H$ be the complement of a path or the complement of a cycle. Suppose that $t$ is the size of the maximum clique minor of $H$. Then the problem of detecting $H$ in an $O(n)$-node graph is at least as hard as finding a $(t-2)$-clique in an $n$-node graph.
\end{restatable}

%\mina{motivation: This idea of making "some" of the partitions a single set can be used with theorem \ref{thm:general-hardness} to have reductions for non-cores.}

\paragraph{Paired Subgraph Isomorphism.}
 In many cases the induced version of the SI problem is much harder than the non-induced version. The simplest example is independent set, when the non-induced version is trivial, whereas the induced version is the hardest pattern detection problem. 
The non-induced version of SI asks for a given pattern $H$ and a host graph $G$, if some supergraph of $H$ is an induced subgraph of $G$. Thus, intuitively the reason why the non-induced version is easier is because there are more options of what subgraph one can return.

We explore this power of allowing an algorithm to return one of a {\em set of possible patterns}. This version of SI has practical applications as well: in  the analysis of social networks for instance, one might be interested in finding some small dense pattern signifying, for instance, a cluster of connected entities, but which dense pattern it is, it might not matter too much.

In graph theory applications related to graph coloring, one is often concerned with $\{H,F\}$-free graphs for various patterns $H$ and $F$ (e.g. \cite{KarthickM18,DabrowskiP18,DabrowskiDP17}). Recognizing such graphs is thus of interest there as well. 

The main question we are interested in addressing is, given two patterns $H$ and $F$, when is it easier to detect either an $H$ or an $F$, than detecting each individual one of $H$ or $F$ separately?

We begin with the case of paired $3$-node patterns. We show that the Paired Pattern Detection problem is in $O(n^2)$ time for every pair of $3$ node patterns and any $n$ node host graph. Moreover, for all but two pairs of patterns, it is actually in linear time.

We then focus on pairs of $4$ node patterns. Similarly to the $k=3$ case, we show that Paired Pattern Detection for any pair of $4$-node patterns is solvable faster than finding $4$-cliques. In particular, $4$-node Paired Pattern Detection is in $\tilde{O}(n^\omega)$ time where $\omega<2.37286$ \cite{almanv21} is the exponent of matrix multiplication, whereas the fastest known algorithm for $4$-clique runs in supercubic, $O(n^{\omega(1,2,1)})$ time where $\omega(1,2,1)\leq 3.252$ \cite{GallU18} is the exponent of multiplying an $n\times n^2$ by an $n^2\times n$ matrix.

An interesting question is then: 
\begin{center}{\em For what pairs can we solve $4$-node Paired Pattern Detection faster than matrix multiplication time}?\end{center}

We give the following general hardness result.

\begin{restatable}{theorem}{setdetectioncore}
\label{thm:set-detection-cor}
Let $S$ is a set of patterns such that every $H\in S$ contains a $k$-clique. Then detecting whether a given graph contains some pattern in $S$ is at least as hard as $k$-clique.
\label{thm:cliqueset}
\end{restatable}

The theorem is a consequence of a more general theorem that we prove by extending
 Theorem \ref{thm:general-hardness}. Theorem \ref{thm:set-hardness} says that we can reduce detecting the core of one of the patterns in a set $S$ to detecting $S$. We also explain how to find such pattern.
\begin{restatable}{theorem}{sethardness}
\label{thm:set-hardness}
Let $G$ be an $n$-node host graph and let $S$ be a set of patterns. There is a pattern $H\in S$, with core $C$ such that one can construct an $O(n)$-node graph $G^*$ in $O(n^2|V(H)|^2)$ time where $G$ has a copy of $C$ as a subgraph if and only if $G^*$ has a copy of a pattern in $S$ as a subgraph.
\end{restatable}

In the context of $4$-node patterns, Theorem~\ref{thm:cliqueset} means that our $\tilde{O}(n^\omega)$ time algorithm for $4$-node Paired Pattern Detection is optimal for any pair of patterns that both contain a triangle or both contain a $3$-independent set $I_3$, under the popular hypothesis that triangle detection requires $n^{\omega-o(1)}$ time.

% -> in applications we might be happy with one of a small set of patterns. in theory recognizing $\{H,F\}$-free graphs is important (give citations); finally non-induced says that we are happy to find any supergraph of $H$, whereas induced only wants $H$. A scenario between induced and non-induced is having a set of admissible patterns.

Thus, to obtain a faster running time, we need to look at patterns $H,H'$ that don't both contain a triangle or an $I_3$.
An interesting case is when $H'$ is the complement of $H$. 

A Ramsey result that follows from Erd\"{o}s and Szekeres~\cite{erdosramsey}
 and made algorithmic by Boppana and Halld{\'{o}}rsson~\cite{BoppanaH92}  shows that in linear time for any $n$-node graph, one can find either a $\log(n)$ size independent set or a $\log(n)$ size clique.
 Thus, for every constant $k$ and large enough $n$, there is a linear time algorithm that either returns a $k$-clique or an $I_k$.
 
 The Ramsey result cannot be extended to show that for every $H$ either $H$ or its complement $\bar{H}$ exists in large enough graphs-- e.g. if the host graph $G$ is an independent set, and neither $H$, nor $\bar{H}$ is an independent set, then neither $H$, nor $\bar{H}$ appears in $G$. Nevertheless, there could still be a fast algorithm that detects whether $H$ or $\bar{H}$ exists in $G$.

Indeed, we show that for $4$ node patterns $H$ there is an $O(n^2)$ time algorithm that does this.

\begin{restatable}{theorem}{complement}
\label{thm:complement}
There is an $O(n^2)$ time algorithm that solves Paired Pattern Detection for $\{H,\bar{H}\}$ for any $4$-node $H$.
\end{restatable}

Our theorem above reinforces the intuition that what makes paired patterns hard to detect is having a common subgraph that is hard. 

We next focus on a different special case of $4$-node Paired Pattern Detection.
% We know that SI for any $4$-node pattern containing a triangle is at least as hard as triangle detection, and thus likely requires $n^{\omega-o(1)}$ time.
A graph pattern detection problem that has been studied a lot
 is that for $4$-Cycle. While non-induced $4$-Cycle detection is known to be solvable in $O(n^2)$ time~\cite{non-induced-4cycle,evencycles}, the fastest known algorithm for the induced version of the problem~\cite{williams2014finding} runs in $O(n^\omega)$ time, the same as for triangle detection. Meanwhile, the $4$-cycle does not contain a triangle or a $3$-independent set, and
 there are no conditional lower bounds that can explain the lack of better than $O(n^\omega)$ time algorithms. It is unclear why the induced case is harder.
 
If $C_4$ detection is at least as hard as $3$-clique, one might expect that the Paired Pattern Detection of $4$-clique (or any pattern containing a $3$-clique) and $C_4$ would still need triangle detection time (this is only intuition, not a formal statement). However, we show that for any $H$ containing a triangle, finding one of $H$ or $C_4$ can be done in $O(n^{7/3})$ time, faster than the current matrix multiplication time $O(n^{2.37286})$ \cite{almanv21}. 


% **********

% pattern set motivation: (1) in coloring they care a lot about induced $\{H,F\}$ free graphs for small subgraphs $H,F$. (2) something between induced and non-induced.

% say about psi, stoc paper, the strongish clique conjecture paper.


% On the algorithm side, we focus on small sized patterns. More specifically, we focus on the $4$-Cycle, and we show fast algorithms for detecting induced $\{C_4,H\}$ for any $H$ containing a triangle. 

\begin{restatable}{theorem}{cfourgeneral}
\label{thm:c4-general}
The Paired Pattern Detection problem for $\{C_4,H\}$ in $n$-node host graphs is in $O(n^{7/3})$ time for any $H$ that contains a triangle, and in $O(n^2)$ time for such $H$ that is not a diamond or $K_4$.
\end{restatable}


% The reason we focus on $C_4$ is that the exact time complexity of detecting an induced $C_4$ is not known. It has an algorithm with triangle detection time but it is open whether there is an algorithm of time $O(n^2)$, which is the running time of detecting a not necessarily induced $C_4$. It might also be the case that there is a reduction from triangle detection to induced $C_4$ detection. Hence our algorithms are important for two reasons: \mina{the following needs paraphrasing}

Detecting a non-induced $C_4$ is equivalent to detecting an induced copy of one of $\{C_4,diamond,K_4\}$, a Set Pattern Detection problem. Thus the Paired Pattern Detection problems
for $\{C_4,diamond\}$ and $\{C_4,K_4\}$ detection are inbetween induced and non-induced $C_4$ detection. Our Theorem~\ref{thm:c4-general} shows that their complexity indeed is inbetween the induced and non-induced $C_4$ detection, and in fact they seem truly easier than induced $C_4$, even though both diamond and $K_4$ are known to be $n^{\omega-o(1)}$-hard from triangle detection.

% Moreover, so far the hardness of patterns are due to having a large clique or independent set implemented in them as a subgraph or as a minor in their core, so we have a "clique" type hardness or an "independent set" type hardness. These algorithms suggest that the only source of hardness of induced $C_4$ cannot be of the "clique" type, since then we would expect to have a reduction from triangle detection to induced $\{C_4,diamond\}$ and induced $\{C_4,k_4\}$ detection using techniques from Theorem \ref{thm:set-hardness}. So we might not expect to have a reduction from triangle detection to induced $C_4$-detection.
    
    It is natural to try to explain the lack of faster than $O(n^\omega)$ time algorithms for $C_4$ by reducing from triangle detection. So far such attempts have failed. Our fast algorithms for paired pattern detection in Theorem~\ref{thm:c4-general} give some explanation for this failure.
    
    Suppose given a host graph $G$, there is a reduction from triangle detection $G$ to induced $C_4$ detection in a graph $G^*$. Our faster-than-triangle-detection-time algorithms for induced $\{C_4,H\}$ detection imply that $G^*$ cannot be $H$-free for any $4$-node $H$ that contains a triangle.
    In particular this is true for $H$ being a $4$-clique and a diamond which are both supergraphs of $C_4$.
    
    First, all reductions from triangle detection so far work for the non-induced version of SI, and non-induced $C_4$ detection is already solvable in $O(n^2)$ time so no higher hardness can be obtained for it. Secondly, all the current lower bound reductions to $H$-detection produce an $H$-partite graph\footnote{An $H$-partite graph $G$ for $k$-node $H$ is an $n$-node graph with its vertices partitioned into $k$ parts $V_1,\ldots,V_k$ and so that if $(i,j)$ is not an edge in $H$, then there are no edges in $G$ in $V_i\times V_j$.}. If we use techniques with this property for induced $C_4$, then the reduction graph $G^*$ in the supposed reduction from triangle detection detection cannot be $C_4$-partite, since $C_4$-partite graphs are triangle free and hence they are also diamond and $K_4$-free.

%\mina{also maybe that when you pair patterns they become easier in the induced case.}

% We also extend Ramsey theoric results for detecting clique or independent sets as follows.

% \begin{theorem}
% \label{thm:complement}
% For any $4$-node pattern $H$, there is an algorithm for induced detection of $\{H,\bar{H}\}$ in an $n$ node host graph that runs in $O(n^2)$ time.
% \end{theorem}

% motivation: The above result suggests that patterns with different sources of hardness tend to offset each other. 


%\mina{maybe say that our proofs might seem case analysis, but this is not surprising as the proof of $P_4$ detection is similarly case analysis.}

%\mina{using the following lemma, we can probably say how the potential reduction graph of triangle to $C_4$ can be, so that it doesn't work for the set case: The reduction graph cannot be $C_4$-partite. Because then we can reduce triangle to $K_4,C_4$ using the same graph: if there is a triangle, by the reduction there is a $C_4$. There can be no $K_4$ in the graph, so if there is a pattern it it $C_4$, and by the reduction we can a triangle. So unlike all the other reductions, it cannot be $C_4$-partite. It cannot be a $k_4$-free graph eiher. }

%\mina{we do cycle and patterns with triangle, $H$ and complement. this is the first set detection (?)}\mina{more motivation: this is like testing a theory on the source of hardness of patterns.}

%We want show that when the source of hardness of two patterns are different, they can be detected faster in a set than individually, and when it is the same, their set detection is hard as well. For the latter, we use a lower bound. For the former, we show the theorem below. 


%\begin{theorem}
%\label{thm:complement}
%For any $4$-node pattern $H$, induced detection of $\{H,\bar{H}\}$ can be done in $O(n^2)$ time.
%\end{theorem}

%The only pattern with no tight algorithm is $C_4$, and there is a gap between the known induced algorithm and non-induced algorithm for $C_4$ detection. We guess that its hardness source is triangle (let's assume we have two hardness sources: clique and independent set). To explore the source of hardness of $C_4$ more, we combine it with patterns that have triangles. We see that for all of these patterns except $k_4$, we can detect $C_4,H$ faster than triangle time. 


==> prelim.tex <==
\section{Preliminaries}

We define $N_G(v)$ as the set of neighbors of $v$ in $G$. We drop $G$ when it is obvious. For a set $S\subseteq V(G)$, we denote by $N_S(v)$ the set of neighbors of $v$ in $G$ that are in $S$.
